A Requirements-Driven Platform for Validating Field Operations of Small Uncrewed Aerial Vehicles

Flight-time failures of small Uncrewed Aerial Systems (sUAS) can have a severe impact on people or the environment. Therefore, sUAS applications must be thoroughly evaluated and tested to ensure their adherence to specified requirements, and safe behavior under real-world conditions, such as poor weather, wireless interference, and satellite failure. However, current simulation environments for autonomous vehicles, including sUAS, provide limited support for validating their behavior in diverse environmental contexts and moreover, lack a test harness to facilitate structured testing based on system-level requirements. We address these shortcomings by eliciting and specifying requirements for an sUAS testing and simulation platform, and developing and deploying it. The constructed platform, DroneReqValidator (DRV), allows sUAS developers to define the operating context, configure multi-sUAS mission requirements, specify safety properties, and deploy their own custom sUAS applications in a high-fidelity 3D environment. The DRV Monitoring system collects runtime data from sUAS and the environment, analyzes compliance with safety properties, and captures violations. We report on two case studies in which we used our platform prior to real-world sUAS deployments, in order to evaluate sUAS mission behavior in various environmental contexts. Furthermore, we conducted a study with developers and found that DRV simplifies the process of specifying requirements-driven test scenarios and analyzing acceptance test results

==> IGNORE.tex <==
\section{Experimental Evaluation} 
\label{sec:sim_eval}

For our second case, we deployed four Hexacopter sUAS in support of a live search-and-rescue demonstration at a beach area in collaboration with emergency responders and lifeguards. While there were no external safety assessors, the public nature of the demonstration, and the fact that it was conducted during the summertime at a crowded beach area, led us to construct a safety case and perform rigorous testing before deployment. The demo enacted the scenario in which a report was received of a missing child, potentially swept out into the water. The sUAS were assigned a search area and dispatched to search, utilizing onboard computer vision, and streaming video when a potential sighting was made. In particular, we wanted to simulate the exercise in advance, to evaluate the impact of windy conditions coming off the water, and to ensure that the following critical safety properties held throughout the mission. In this case, all three were considered safety-related, with C2.1 and C2.2 directly related to flight safety, and one C2.3 related to avoiding informational overload which is considered a situational awareness demon~\cite{ensley1995toward}.



\begin{enumerate}[label=C2.\arabic*,leftmargin=25pt]
     \item No search flights shall be conducted over the beach.   \textit{Validation:} 
     {\small\texttt{sUAS location in the environment (lat, long, alt) $\cap$  No-Fly Zones (lat, lon, alt) = $\phi$}}
    \item No sUAS will land in the water or on the beach. All landings must be at home location \textit{Validation:} {\small\texttt{if alt <= |1m|} then  Distance sUAS(lat,lon) sUAS(home.lat, home.lon) ALWAYS $<$ 8m }
    \item sUAS must perform a ``safe'' takeoff during the mission maintaining both lateral and altitude distance.  (Note: This scenario is different from maintaining lateral distance in flight, because launch areas are often space-constrained, meaning that sUAS must stagger their takeoffs if they are positioned too closely together.) \textit{Validation:} {\small\texttt{(Distance sUAS1(lat,lon) sUAS2(lat,lon) ALWAYS > 8 meters) AND (Distance sUAS1(lat,lon,alt) sUAS2(lat,lon,alt) ALWAYS > 20 meters) WHEN Mode(sUAS1)=Takeoff AND Mode(sUAS2)=Takeoff} (for each pair of sUAS)}
    
    \item Routes must be completed successfully in winds up to 23mph. There are many ways to measure a successful mission, and for this one we establish a baseline for the duration of the mission with Winds = 0 mph as a comparison. \textit{Validation:}{\small\texttt{MissionDuration when (WINDS =  Xmph) <= (MissionDuration * 1.25) when (WINDS= 0 mph) AND for each Waypoint in Mission sUAS flies within 1 meter.}}
\end{enumerate}


\subsection{Addressing the Research Questions}
We address RQ1 and RQ2 by examining the outcomes of our use cases. 

\subsubsection{RQ1: Support for Diverse Tests} To address RQ1 we applied \DW to two planned real-world deployments. As an initial step for each scenario we created a realistic configuration that included a 3D map of the designated area, no-fly zones, wind and lighting conditions, and enabled direct human input to control an sUAS. Table \ref{tab:briar-test} summarizes the test configuration for UC\#1, and Table \ref{tab:mc-test} for UC\#2.
\input{tables/tab_BRIAR_test}
\input{tables/tab_MC_test}

We identified critical safety requirements for each deployment and translated them into checkable properties supported by \DW. All of the specified properties were supported in \DW. Tests were executed successfully and the outcomes were displayed to the user. On the other hand, as depicted in Table \ref{tab:factors}, we have only integrated a subset of the potential configuration parameters in the current prototype. For example, we have not yet integrated any form of sUAS fault injection,  GNSS (satellite) or wireless network failures. We therefore deliberately did not attempt to configure the environment with these properties. Regardless of these limitations, \DW allowed us to test some important scenarios.

\subsubsection{RQ2: Ability to detect problems}
To address RQ2 we executed a series of tests for each of the scenarios. We deliberately included test cases that we expected to fail in order to evaluate \DW's ability to raise errors appropriately. Here we report one example from each of the use cases. In Figure \ref{fig:wind} we plot flight logs from simulations in winds of 23mph and 30mph. The first test passed whilst the second one (at 30mph) failed when the sUAS blew away into the lake. Second, in Figure \ref{fig:griffiss} we show several no-fly zones at the airport. In this example, a flight triggered a FAILED TEST because the flight path flew over a temporary no-fly zone violating C1.2. These and many other examples, demonstrated that \DW was able to accurately differentiate between PASSed and FAILed test cases.

\begin{figure}
    \centering
    
    \begin{subfigure}{0.52\columnwidth}
  
    \includegraphics[width=\columnwidth]{figures/flightlogs/MC-Wind23.PNG}
    \footnotesize{
     Wind speed:~~~~{\it \ul{23 mph}}  \\
     Duration:~~~~~~~{\it 19 mins, 39 secs} \\     Dist. flown:~~~~{\it 1.29 km} \\
     Outcome:~~~~~~~{\it Passed}
     }
    \end{subfigure}
     \begin{subfigure}{0.45\columnwidth}
    \includegraphics[width=\columnwidth]{figures/flightlogs/MC-Wind.PNG}
     \footnotesize{
     Wind speed:~~~~{\it \ul{30 mph}}  \\
     Duration:~~~~~~~~{\it 13 mins, 6 sec} \\     Dist. flown:~~~~~{\it 1.46 km} \\
     Outcome:~~~~~~~{\it Blown into lake}
     }
    \end{subfigure}
  
    \caption{Flight test passes when winds were $\approx$ 23 mph but unsurprisingly failed at 30 mph. No properties were violated in the low-wind example, but property C2.4 was violated in the high-wind scenario.}
    \label{fig:wind}
    \vspace{9pt}
    
 
    \begin{subfigure}{\columnwidth}
  
    \includegraphics[width=\columnwidth]{figures/flightlogs/nofly-example.PNG}
    \end{subfigure}
    
    \caption{A flight is planned (pale blue route) to position a drone for image collection. However, the property checks indicate that it violated case C1.3. by infringing on the no-fly zone (green) established to protect human participants from the direct flight path.  Outcome: FAIL}
    \label{fig:griffiss}
\end{figure}

==> OLD_sec_06_eval_uc1_backup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% !!!  OLD DO NOT USE !!! %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{tables/tab_MC_test.tex}
\noindent\textbf{UC1 -- Video Collection at Pitch and Range:}

For the first use case, a team of computer vision researchers provided a list of requirements for collecting aerial images to the software engineering team for designing sUAS applications to collect aerial images with specific camera pitches and custom flying patterns. The engineering team developed an sUAS application to deploy two sUAS at a test location of an active airbase,  tasked with collecting aerial imagery of people (hired actors) from diverse distances, pitches, and angles. Given the flight patterns of each sUAS, and the vicinity of the three airspaces, there is potential for overlapping flight paths. The test scenario including the environment, sUAS, and mission properties to test are shown in Table \ref{tab:briar-test}.

% The airport authorities have strict flight regulations, the majority of which were already covered by our default safety constraints; however, the following  scenario-specific properties were added. 



% \begin{enumerate}[label=C1.\arabic*,leftmargin=25pt]


%     \item The lateral distance must be maintained between all inflight sUAS at all times.\\ 
%     \textit{Validation:} Minimum lateral distance monitor - 20 meters
%     % {\small\texttt{Distance sUAS1(lat,lon) sUAS2(lat,lon) ALWAYS > 20 meters}} (for each pair of sUAS in air).%YES
    
%     \item The sUAS must not fly over no-fly zones including taxiways, runways, or areas designated as ``actor'' zones.\\ %YES\\
%      \textit{Validation:} 
%      {\small\texttt{sUAS location in the environment (lat, long, alt) $\cap$  No-Fly Zones (lat, long, alt) = $null$}}
%      No Fly Zone Monitor - specified all no fly zones 
%     \item Any sUAS takeoff needs to be immediately aborted when the launch pad is not clear (e.g., humans or birds in the vicinity).\textit{Validation:} 
%     Human Intervention Monitor 
%     {\small\texttt{Human Command = Abort IF (Mode(sUAS1) = Takeoff  AND TargetPos = (lat = sUAS\_lat, long = sUAS\_long, alt $>$ sUAS\_alt))}}
% \end{enumerate}


\noindent\textbf{UC2 -- Search-And-Rescue:}
For our second case, we deployed four Hexacopter sUAS in support of a live search-and-rescue demonstration in collaboration with emergency responders. The public nature of the demonstration, and the fact that it was conducted during the summertime at a crowded beach area, required rigorous testing before deployment. The sUAS were assigned a search area and dispatched to search, utilizing onboard computer vision, and streaming video when a potential sighting was made. In particular, we wanted to simulate the exercise in advance, to evaluate the impact of windy conditions coming off the water, and to ensure that the critical safety properties held throughout the mission. Test scenarios description and configurations are shown in Table~\ref{tab:mc-test}
% In this case, all three were considered safety-related, with C2.1 and C2.2 directly related to flight safety, and one C2.3 related to avoiding informational overload which is considered a situational awareness demon~\cite{ensley1995toward}.

\begin{figure}
    \centering
    
    \begin{subfigure}{0.46\columnwidth}
  
    \includegraphics[width=\columnwidth]{figures/flightlogs/MC-Wind23.PNG}
    \footnotesize{
     Wind speed:~~~~{\it \ul{23 mph}}  \\
     Duration:~~~~~~~{\it 19 mins, 39 secs} \\     Dist. flown:~~~~{\it 1.29 km} \\
     Outcome:~~~~~~~{\it \texttt{PASSED}}
     }
    \end{subfigure}
     \begin{subfigure}{0.40\columnwidth}
    \includegraphics[width=\columnwidth]{figures/flightlogs/MC-Wind.PNG}
     \footnotesize{
     Wind speed:~~~~{\it \ul{30 mph}}  \\
     Duration:~~~~~~~~{\it 13 mins, 6 sec} \\     Dist. flown:~~~~~{\it 1.46 km} \\
     Outcome:~~~~~~~{\it Blown into lake}
     }
    \end{subfigure}
  
    \caption{Flight test passes when winds were $\approx$ 23 mph but unsurprisingly failed at 30 mph (Violating C2.3 described in Table \ref{tab:mc-test})}
    \label{fig:wind}
    \vspace{9pt}
    
 
    \begin{subfigure}{\columnwidth}
  \centering
    \includegraphics[width=0.8\columnwidth]{figures/flightlogs/nofly-example.PNG}
    \end{subfigure}
    
    \caption{A flight is planned (blue route) to position an sUAS for image collection. However, the flight violated case C 1.2 described in Table \ref{tab:briar-test} by infringing on the temporary no-fly zone (green).  Outcome: \texttt{FAILED}}
    \label{fig:griffiss}
    \vspace{-15pt}
\end{figure}

% \begin{enumerate}[label=C2.\arabic*,leftmargin=25pt]
%      \item No search flights shall be conducted over the beach.   \textit{Validation:} 
%      {\small\texttt{sUAS location in the environment (lat, long, alt) $\cap$  No-Fly Zones (lat, lon, alt) = $\phi$}}
%     \item No sUAS will land in the water or on the beach. All landings must be at home location \newline \textit{Validation:} {\small\texttt{if alt <= |1m| then  Distance sUAS (lat, lon) sUAS(home.lat, home.lon) ALWAYS $<$ 8m }}
%     \item sUAS must perform a ``safe'' takeoff during the mission maintaining both lateral and altitude distance.  (Note: This scenario is different from maintaining lateral distance in flight, because launch areas are often space-constrained, meaning that sUAS must stagger their takeoffs if they are positioned too closely together.) \textit{Validation:} {\small\texttt{(Distance sUAS1(lat,lon) sUAS2(lat, lon) ALWAYS > 8 meters) AND (Distance sUAS1(lat, lon, alt) sUAS2(lat, lon, alt) ALWAYS > 20 meters) WHEN Mode(sUAS1)=Takeoff AND Mode(sUAS2)=Takeoff} (for each pair of sUAS)}
    
%     \item Routes must be completed successfully in winds up to 23mph. There are many ways to measure a successful mission, and for this one we establish a baseline for the duration of the mission with Winds = 0 mph as a comparison. \textit{Validation:} {\small\texttt{MissionDuration when (WINDS =  Xmph) <= (MissionDuration * 1.25) when (WINDS = 0 mph) AND for each Waypoint in Mission sUAS flies within 1 meter}}
% \end{enumerate}


\subsection{Addressing the Research Questions \& Discussion}

%\subsubsection{RQ1: Support for Diverse Tests}
\subsubsection{\textbf{Ability to configure real-world requirements}}
We applied \DW to the planning and validation of two real-world deployments of our own DSuT. We created a realistic configuration that included a 3D map of the designated area, no-fly zones, wind, and lighting conditions, and enabled direct human input to control an sUAS. Tables \ref{tab:briar-test} and \ref{tab:mc-test} summarize the test configuration for UC1 and UC2.
We identified critical safety requirements for each deployment and translated them into test properties supported by \DW. 

% The primary cost and effort in setting the environment up for each use case was in writing Python programs to check the additional monitorable properties defined in the test specifications. However, we observed that these properties are likely to recur over multiple scenarios, meaning that monitors are reusable and can easily be templated and then populated with mission-specific values. 

% Connecting our DSuT to \DW was otherwise simple, and required us to modify one connection string for each sUAS so that it connected to \DW instead of to a physical sUAS or to Gazebo, our previously used simulator. 

The missions flown in \DW were ones that we were already planning for the two deployments, and were specified entirely using our own DSuT. Tests were then executed successfully and the outcomes were displayed to the user. However, as depicted in Table~\ref{tab:factors}, we have only integrated a subset of the potential configuration parameters in the current prototype. For example, we have not yet integrated any form of sUAS fault injection, GNSS (satellite), or wireless network failures. We, therefore, deliberately did not attempt to configure the environment with these properties and leave their inclusion to the next phase of our work. The configuration of real-world scenarios showed that \DW allows configuring sUAS, environmental settings, and tests based on system-level requirements, simulating sUAS in realistic conditions, and analyzing acceptance test results. 

\subsubsection{\textbf{Ability to validate requirements}}
To address RQ2 we executed a series of tests for each of the use cases. We deliberately included test cases that we expected to fail, in order to evaluate \DW's ability to raise errors appropriately. Here, we report one example from each of the use cases. In Figure~\ref{fig:wind} we plot flight logs from simulations in winds of 23mph and 30mph. The first test passed whilst the second one (at 30mph) failed when the sUAS blew away into the lake. Second, in Figure~\ref{fig:griffiss} we show several no-fly zones at the airport. In this example, a flight triggered a \texttt{\small FAILED} test because the flight path flew over a temporary no-fly zone violating C1.2. These and many other examples demonstrated that \DW was able to accurately differentiate between \texttt{\small PASSED} and \texttt{\small FAILED} test cases.






\subsubsection{\textbf{Ability to Identify the Operating Boundaries of sUAS Applications}}
The inclusion of fuzzy testing in the framework allows \DW to compare simulation results across configured and fuzzed test cases automatically. After comparing simulation results, \DW generates acceptance test reports and presents mission analytics on a dashboard. The inclusion of mission analytics information in the Acceptance Test report provides several benefits. First, automated mission analytics relieve developers of the burden of writing custom scripts for analysis simulation logs. Second, comparing fuzzy test results with user-configured tests allows determining the limitations of an sUAS application and the environmental conditions under which it satisfies the system requirements. In order to demonstrate the practical application of including fuzzy testing analysis in acceptance test reports, we conducted an experiment to assess the performance of a drone flying in a circular trajectory at different speeds. The tests were configured to fuzz the wind velocity, with a maximum wind velocity of 18 meters/second. The drone was assigned to fly at velocity of 6, 9, and 13 meters/second, and the results were analyzed to determine its ability to withstand varying wind conditions. Alongside conducting the tests under no windy conditions, \DW generated two additional fuzzy tests for each drone velocity and conducted simulations at 10 and 18 meters/second of wind velocity. 
 Figure \ref{fig:fuzz_results} shows a series of plots generated by \DW monitoring environment to visualize how the increasing wind velocity in the East direction impacts the sUAS's flight path as its velocity increases. The comparison of Figures \ref{fig:drone_speed_6}, \ref{fig:drone_speed_9}, and \ref{fig:drone_speed_13} provides insights into the ability of sUAS to fly circular missions under varying wind conditions. The data show that sUAS is not capable of flying circular missions above 6 meters/s when the wind velocity approaches 18 meters/s. This suggests that the ability of sUAS to perform certain tasks may be limited in environments with high wind speeds. However, the simulation results also indicate that sUAS can withstand wind speeds of up to 10m/s without deviating by more than 5 percent from their flight path and complete the mission. Thus, such analytics offer valuable insights for the development and operation of sUAS amidst uncertain circumstances. Additionally, the data visualizations available on the dashboard aid developers in identifying operational constraints and detecting potential bugs within their applications.
 

% One additional aspect we have partially considered (but does require further research) is introduced by the fidelity, or lack of fidelity, of the underlying physics engine. To trust the results of the simulation, we need confidence that the underlying physics engine and the environmental configuration behave in ways that are very similar to the physical sUAS in the real world. To address this risk, we performed pairwise tests of flights in the simulator vs. the real world and compared the results. We evaluated two simulators -- the inbuilt AirSim physics engine, and Gazebo. 

% As illustrated in the example shown in Figure \ref{fig:fidelity}, but also observed in other flight tests, the Gazebo simulator has higher real-world fidelity than the native AirSim simulator. The difference is quite marked in this example, because the flight uses the flight controller's ``offboard'' mode which requires more advanced features. For purposes of this work, we have however reported AirSim results, as it is seamlessly integrated with the Unreal Engine in which the environment is configured. In future work, we will explore Gazebo integration and/or ways to increase the fidelity of AirSim. Fidelity of the sUAS models is critical to the success of \DW; however, simply using Gazebo alone does not provide the rich environmental data that is provided by the Unreal Engine.





% \ankit{I do agree with the point that Gazebo's physics engine is better than Airsim's, but I think in this particular example, the landing locations are different in Airsim and Gazaebo sim. So, revising the discussion}

\subsubsection{\textbf{Ease of Test Specification in \DW}}
To evaluate the usability of our system for developing test scenarios and configuring test properties for requirements, as well as to determine the effectiveness of our Acceptance Test Report in facilitating developers in understanding and analyzing simulation outcomes, we conducted a preliminary user study with X participants. To recruit participants, we reached out to our personal contacts and invited them to participate in the study. Participant selection criteria included software engineering and testing experience. Each participant was assigned one of three different system-level requirements shown in table Z to test using \DW. Each user study session was finished in approximately 30 minutes. Tables Y provide details on the participants and their industrial software engineering experience. 

% Findings
All participants were able to configure the multi-sUAS test scenario using \DW and draw insights from the provided acceptance test reports. In general, all participants found the user interface for configuring test scenarios to be intuitive and easy to use. Specifically, participant P x expressed very positive feedback regarding the entire ecosystem, suggesting it to be a valuable tool for conducting simulation testing. However, some issues were identified by participants, specific to multiple sUAS simulation, during the study. several participants (two) reported difficulties in specifying the home geolocation of each sUAS in the environment. Specifying the desired home location of sUAS required participants to first copy the geocoordinates from Google Maps and then paste them into the \DW application. This process was cumbersome and time-consuming. In addition, PX, PY, and PZ  also suggested the need for visualizing the geolocation of multiple drones on a 2D map to better understand the relative proximity of each drone to one another prior to the start of the simulation.

While observing the simulation, participants were interested in observing the flight path of all sUAS in the 3D environment. It became challenging for participants to observe the activities of all sUASs at the same time when the sUAS were far apart from each other. This was because the view port of the simulation environment, which could be adjusted and zoomed in/out, was not capable of covering the entire area occupied by all the sUASs simultaneously. This issue emphasizes the need for a solution that supports multi-viewports based on sUAS location in the environment so that users can observe multiple sUAS even when they are far apart. 

Finally, after observing the simulation, participants proceeded to analyze the generated acceptance test report of the configured test scenario. While all participants found the presentation of information in the acceptance test report extremely helpful, particularly the graphical comparison of expected and actual flight paths, several areas for improvement were identified. Firstly, P3 suggested that the test report should include explanations regarding why an sUAS deviated from its flight path. This could include factors such as increased wind velocity, GPS uncertainty, or any sensor malfunction. By providing such explanations, developers would have a better understanding of the factors influencing the sUAS flight paths, and could take appropriate actions to improve the performance of their sUAS application. 

\input{tables/participants}

% Geo Cordinate Pecision
% we will use these feedback and comments to improve the usability ofo the DW platform

% In summary, we can conclude that


\begin{figure*}
  \begin{minipage}[htbp]{.33\linewidth}
    \includegraphics[width=\linewidth]{figures/fuzzy_results/drone_6.png}
    \caption{Caption}%
    \label{fig:drone_speed_6}
  \end{minipage}\hfill
  \begin{minipage}[htbp]{.33\linewidth}
    \includegraphics[width=\linewidth]{figures/fuzzy_results/drone_9.png}
    \caption{Caption}%
    \label{fig:drone_speed_9}
  \end{minipage}\hfill
  \begin{minipage}[htbp]{.33\linewidth}
   \includegraphics[width=\linewidth]{figures/fuzzy_results/drone_13.png}
    \caption{Caption}%
    \label{fig:drone_speed_13}
  \end{minipage}%
  \caption{Part of generated Acceptance Test report showing the operating boundary of sUAS application across varying sUAS velocity and wind velocity}
  \label{fig:fuzz_results}
\end{figure*}





% \subsubsection{Usability of Acceptance Test Report}
% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/plots/mutation_wind_test.png}
%     \caption{As part of the fuzzy testing feature of \DW, the analytics dashboard provides information regarding the impact of incresing wind speed in a particular direction on the flight path}
%     \label{fig:fuzz_result}
% \end{figure}
%%% Stashing original figure down here!





% \begin{figure*}
%     \centering
%     \includegraphics[width=.5\columnwidth]{figures/fuzzy_results/drone_6.png}

% \includegraphics[width=.5\columnwidth]{figures/fuzzy_results/drone_9.png}

% \includegraphics[width=.5\columnwidth]{figures/fuzzy_results/drone_13.png}
%     \caption{As part of the fuzzy testing feature of \DW, the analytics dashboard provides insights regarding the impact of incresing wind and sUAS velocity in a particular direction on the flight path}
%     \label{fig:fuzzy_results}
% \end{figure*}




% \begin{figure}
%     \centering
    
   
%     \begin{subfigure}{0.43\columnwidth}
%   \centering
%     \includegraphics[width=\columnwidth]{figures/flightlogs/nofly-example.PNG}
%     \footnotesize{
%      Flight (blue route) violated case C1.3 by infringing on the temporary no-fly zone (green).  

%     }
%         \label{fig:griffiss}
%     \end{subfigure}
%      \begin{subfigure}{0.53\columnwidth}
  
%     \includegraphics[width=\columnwidth]{figures/flightlogs/MC-WindDebacle.PNG}
%     \footnotesize{
%      Flight test failed with wind = 30 mph, with crash into lake. Property C2.4 was violated.
%      }
%       \label{fig:wind}
%     \end{subfigure}
%   % I'm working on this. give me a minute!!!
% \caption{Two failed tests executed in \DW. The first is taken from UC\#1 and the second from UC\#2.}
%   % HOLD FOR CAPTION HERE>
%     \vspace{-15pt}
% \end{figure}




In response to RQ1, we were able to apply \DW to our two use cases and demonstrate its practical applicability in real-world testing scenarios and integration in a thorough software testing process. We were able to specify the safety requirements, connect our own DSuT with minimal effort, execute test cases and analyze the results provided by the Acceptance Tests to further improve our application. However, the fidelity of the underlying physics engine must be considered before trusting simulation results. While Airsim uses a simplified physics engine for multirotors called Fast Physics, this engine can be replaced with more complex physics engine. For the purpose of this work and to illustrate our approach, we have reported results using Airsim's default physics engine. In the future, we will develop APIs that will allow developers to integrate their own physics engine with the \DW.

In response to RQ2, we found that..

==> OLD_sec_06_eval_uc2.tex <==
%\subsection*{UC \#2: Emergency Response Demo} 


==> OLD_sec_06_evaluation_backup.tex <==
\section{Experimental Evaluation} 
\label{sec:sim_eval}

To demonstrate \DW's applicability to real-world sUAS applications, and its support for testing system-level requirements,  we (i) performed a case study (following the guidelines described by Runeson and Hoest~\cite{runeson2009guidelines}) for two sUAS use cases for which we needed assurances that our DSuT would perform safely in the real world, and (ii) conducted a user study with sUAS developers asking them to configure a multi-sUAS test scenario based on given requirements.
%analyze acceptance test results using \DW, and compare our proposed testing process and infrastructure with their current practices.    


% For the selection and creation of the use cases, we followed the guidelines described by Runeson and Hoest~\cite{runeson2009guidelines}, and explore the following research questions. 
% The main requirements and selection criteria for the use cases were the availability of diverse scenes and environmental conditions, mission-specific test cases, and potential safety risks that needed to be tested and mitigated.
We explore the following research questions: \\
\noindent$\bullet$ \emph{RQ1: }\emph{Can \DW be used for defining and executing realistic test scenarios, and what is the effort required for creating and specifying them?}
    
     We first applied \DW to two distinct real-world sUAS application scenarios, creating a series of acceptance tests for each of them, and specifying environmental features and respective monitors relevant to the tests to determine the feasibility of our approach. 
     Second, through our user study, we asked sUAS developers to configure real-world scenarios using \DW to estimate the effort it takes to set up a test scenario, and to understand the quality and usefulness of test reports that \DW generates.  
    % \vspace{-0.9em}
    
    \noindent $\bullet$ \emph{RQ2: }\emph{Can we detect problems and safety-related issues by executing our test scenarios using the \DW testbed?} 
    We address this RQ by running a series of simulations in our \DW platform, based on the aforementioned tests. We further introduce a series of seeded ``faults'' causing failures in the system and assess if \DW is capable of detecting and documenting them during the course of a simulation run.
    
    % \vspace{-0.9em}
    
    % \noindent $\bullet$ \emph{RQ3: Are the results obtained from the simulator representative of those expected in the physical world?} We address this RQ by carefully devising tests that represent diverse sUAS tasks and environmental conditions, and then comparing simulation results against results obtained from tests using physical sUAS.
    
    % \jch{Actually the one results I have shows AIRSIM isn't that accurate. Gazebo is much more accurate!!  I think we should mention that in threats instead of in RQ3 or where I have it now.}
  


% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/Simulation/boston-flight-1.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
    



\subsection{\DW Prototype Implementation}
We implemented an initial prototype to support Pixhawk/PX4 application tests for a number of environmental configuration options and monitorable properties.
The configurable properties and features currently supported are marked as implemented (or partially implemented) in~\citetable{factors}.
% , and implemented monitors are described in Table~\ref{tab:monitors}. 

We developed a web application using the React Web framework that allows users to interact with \DW. The web application has a Wizard that guides users through the process of creating a test scenario, as well as a dashboard that displays the consolidated simulation results for users to analyze. 
% The screenshots of the web application are shows in Figure \ref{fig:sim_ui}. 
Through the web application, users can configure their sUAS, environment, and test properties, which are then sent to the backend server written in Python using Flask over HTTP. Using the configuration provided by the user, the back-end server generates the fuzzy test scenario and instantiates the simulation environment. 

Our \DW simulation environment was implemented using the Unreal Engine~\cite{unrealengine}, integrating open-source digital shadow models of the real world by using Cesium for Unreal~\cite{cesium}. We simulated sUAS using AirSim~\cite{shah2018airsim}, an open-source, cross-platform simulator, and used AirSim's APIs to simulate weather conditions in the environment.

Furthermore, we implemented runtime monitors as Python modules that collect data (e.g., using AirSim's APIs) associated with test properties specified by the user. Additionally, interaction data is collected through input devices such as handheld controllers, keyboards, and game controllers. Finally, ``Unreal Blueprints'' and Airsim APIs were used to monitor the changes in the environment as well as the activities of actors such as pedestrians. 

%Unreal Blueprint is a visual scripting technology that allows us to monitor and control every element in the Unreal Environment, recording a corresponding timestamp for each collected information. This is later vital for consolidating the data based on timestamps and generate the final test report. 

% We currently provide a textual output of test results on the command line of the monitoring and simulation environment and in a log report. However, we are concurrently developing a proper dashboard to provide visual (runtime) information and live updates to the user during test execution.



\subsection{Drone System Under Test}
Both use cases are enacted using our own semi-autonomous, multi-sUAS system, which includes a Ground Control Station (GCS) supported by a suite of microservices, onboard autonomous processing capabilities, and diverse GUIs to support human interactions. The Onboard Pilot acts as an application layer for the PX4 autopilot stack which includes flight control software and hardware for executing plans. Its internal \textit{State Machine} receives mission specifications and instantiates itself dynamically for the current mission. It then uses its onboard state machine to progress through a series of tasks, with transitions triggered by events detected from its own sensor data and/or messages received from the GCS or other sUAS.

The ground control station uses microservices and a publish-subscribe architectural style~\cite{muccini2018iot}, with each microservice providing a specific capability such as airspace leasing, multi-sUAS coordination, or runtime monitoring. Finally, graphical and hardware user interfaces enable human-machine interactions. Most of the interactions are GUI-based; however, in case of emergency, humans can directly issue commands via handheld radio controllers. The GUI components are built on a centrally hosted {\it web application} that asynchronously sends and receives status data and video streams over a Mesh Radio via GCS's message broker and the onboard pilot modules.

\input{tables/tab_BRIAR_test}

\subsection{Use Case Driven Test Scenarios}
We focused our experiments on two real-world use cases. The first use case represents the deployment of multiple sUAS in September 2022 at an active airbase to collect long-distance imagery of people at diverse pitches and altitudes, and the second use case involved a live search-and-rescue demonstration that we conducted in August 2022 in conjunction with a local Fire Department's water-rescue team. We provide details for each use case including the environmental configurations and unique requirements that led to customized test properties.

\input{sec_06_eval_uc1}

\input{sec_06_eval_uc2}










% \simpleitem{Research Design:}
% For each of the use cases, we followed the following process of exploring the different scenarios, designing the tests (RQ1), specifying the test setup, executing the simulations, and finally, analyzing the results (RQ2).  


% Just mapping out a plan here...
% \begin{enumerate}
%     \item Explore scenarios (to make this more about 'requirements' and avoid the 'testing' reviewers I think we should provide actual use case scenarios)
%     \item Design test contexts with some variability (fuzzing??) so that we can run mutants
%     \item Add mission-specific properties as needed to the default ones.
%     \item Design missions for each scenario (e.g., flight routes, coordination handlers etc etc)
%     \item Execute simulation and check for violations of safety constraints.
% \end{enumerate}

% Something about running STRESS tests in the simulator and real tests under 'normal conditions in the real world.

% But we also need to demonstrate some results.  We could show how these results served as evidence in the safety case that was acceptable to nuair (Griffiss). We could collect some numbers.





% \subsection{RQ1 -- Application of \DW}


% \subsection{RQ2 -- Simulation}



% \subsection{Discussion}

% \subsection{Fidelity Testing}
% Short section on fidelity testing. 


==> backup_impl_text.tex <==
\section{Acceptance Testing & \DW Implementation}





\subsection{Acceptance Tests}




\subsection{APIs for System Testing}
Given that the primary goal of \DW is to empower users to test diverse sUAS applications within various mission contexts, we also created several well-defined APIs which allow sUAS applications under test to interact with \DW. The APIs include the following:

\begin{itemize}[leftmargin=*]
    \item[-] \emph{Configuration API: } \DW provides end-users and developers with the ability to configure the environment and properties to be monitored. As an input, \DW accepts a JSON file structured as shown in Listing \ref{lst:Env-config} and Listing \ref{lst:monitor-config} to configure the simulation environment and monitor simulation results. 
    
    \item[-] \emph{Application  Interface: } 
    In the sUAS software application development, the control commands are sent to the autopilot firmware, such as PX4, which generates the corresponding actuator signal and forwards it over a UDP or TCP connection to the simulator. Through DW, end-users can specify a unique port for each sUAS in the simulation to exchange data with the firmware, allowing seamless multi-sUAS simulations. 
    
    \item[-] \emph{Human Interaction Interface:} For the purpose of debugging and identifying the impact of human intervention on the run time behavior of autonomous sUAS, \DW provides a virtual controller interface written in Python, which can be used to send control commands such as Take-off and Land or to switch sUAS modes. The virtual controller implementation may also be extended to physical controllers, as long as each key on the physical controller has a Python binding interface available.
    
    \item[-] \emph{Simulation Data Subscription Service: } Finally, in order to enable developers to develop their own custom monitors, \DW publishes run-time monitoring data over MQTT topics to which developers can subscribe to monitor information about sUAS, environment, and human interactions. 
   
\end{itemize}

\subsection{Implementation}

For experimentation purposes with \DW (cf.~\citesec{evaluation}), we implemented an initial prototype to support Pixhawk/PX4 application tests for a number of environmental configuration options and monitorable properties.
The configurable properties and features currently supported are marked as implemented (or partially implemented) in Table \ref{tab:allprops}, and  monitors are further described in ~\citesec{evaluation}.
Our \DW simulation environment was implemented using the Unreal Engine~\cite{unrealengine}, and  integrated open-source digital shadow models of the real world by using Cesium for Unreal~\cite {cesium}, a plugin for the Unreal Engine, to visualize and integrate high resolution, real-world, photogrammetry and 3D models.
For simulating sUAS we use  AirSim~\cite{shah2018airsim}, an open-source, cross-platform simulator for drones and several other types of (ground-based) vehicles. This decision was deliberately made as  AirSim is the only simulator that integrates with the Unreal Engine, and uses the PX4 flight controller stack on which our own DSuT is built. Furthermore, we leveraged the APIs provided  by AirSim to simulate weather conditions in the environment, such as wind, fog, and snow. The simulation initialization manager component thereby instantiates multiple sUAS in the digital shadow of the real world and configures the environmental conditions as described in the test specifications. 
%\input{listings/env_config}

Finally, to collect, analyze, and validate the runtime behavior of sUAS and human interactions  \DW monitors were implemented as independent Python modules. These Python modules were configured and activated according to the test properties specified in the JSON file. To collect the different types of information necessary for validation three main types of monitors were implemented and used. First, monitors developed to capture the run-time behavior of suAS utilize Airsim's simulator APIs to directly connect to the (simulated) sUAS and to query data. Second, the human interaction monitor established a connection with the input devices, such as UIs, RC handheld controllers, keyboards, or game controllers, to record human interactions during mission execution. Finally, we used ``Unreal Blueprints'' to monitor the changes in the environment as well as the activities of a specific actor in it. For example, a drowning victim or an escaping suspect. Unreal Blueprint is a visual scripting technology that allows us to monitor and control every element in the Unreal Environment, recording a corresponding timestamp for each collected information. This is later vital for consolidating the data based on timestamps and generate the final test report. The test report provides two key insights. First, the consolidated information at the mission level from each sUAS in the environment, including any changes to the 3D environment. Second, it reports if any of the test properties were breached during the mission. Therefore, the test report serves as a critical artifact to diagnose the SuT.


% and  with multi-sUAS flight in order to provide reusable, high-fidelity, and realistic flying environments and conditions that support software engineers in rapid, incremental validation of their own systems deployed on realistic missions within real-world environments prior to executing field-tests with physical sUAS. 







%%% mission level log->
%%% combine information from the different plugins/ shadow models  - tells us which drone have collided with what , where, why....

==> box_req.tex <==
\noindent\mybox{lightgray}{{
\noindent {\bf Requirement ID:~} UAV-121\\
% \noindent {\bf Test Name:~} Test mission in windy conditions\\
\noindent {\bf Description:~}``A team of sUAS shall successfully complete a mission consisting of a series of waypoints in wind conditions of 23 mph for altitudes above 30ft AGL.''\\
{\bf Real-World Environmental Specifications~}\\
{\bf 1:} mission=MSN-1\\
{\bf 2:} (wind=15mph, $0<ALT<30ft$ AGL) \&\& (wind = 23mph,$ALT>30ft$ AGL)\\
{\bf 3:} (Region=Boston Downtown) \&\& (UAV Home=(42.358564, -71.057413))}}\\[1ex]

%%mv: probably state-driven pattern if we go with ears?
%% something along
% While executing a mission... a team of  sUAs shall reach  its predefined waypoints - within x-meters, and shall maintain a minimum distance to the ground of 40ft? 
%what does "successfully complete" mean? (reach all waypoints?) - which would be the acceptance criteria
%%%% 

==> discussion.tex <==
\section{Testing the Simulator}
% \jch{Ankit -- this is so important that I suggest you pull out the parts about testing the simulator from the conclusions and put it into its own (SHORT) section.}
The utility and effectiveness of a simulator is limited by its fidelity. In this Chapter we have focused on creating real-world environments in which UAV system tests can be performed. However, n\"aively trusting in the fidelity of the simulation environment can introduce new types of problems, and create false confidence that a UAV system will execute correctly in real-world conditions \cite{dahlstrom2017fidelity}.  It is therefore imperative to test the fidelity of the simulator itself. We therefore lay out a simple testing roadmap as follows:

First, The formal validation of the effectiveness of the framework is challenging because (a) flying UAVs in extreme weather conditions, such as strong winds over 30 mph poses significant risks to public safety, and (b) it is not feasible to recreate very specific scenarios of emergency response, such as multiple UAVs scouting in the middle of a city to detect a fire. To address this challenge, a comparison of simulation results with the corresponding real-world vignette test will be conducted to gain insights regarding the usefulness of the framework in UAV software development. 

Second, we aim to create simulation tests automatically based on our initial framework to ensure the robust run-time behavior of the UAV. Specifically, we are planning to employ the metamorphic test paradigm \cite{segura2018metamorphic}, in which various properties of the environment will be randomly inserted or removed from our simulation in order to test the UAV behavior in unique environmental conditions. Such methodologies would enable evaluation of the UAV software against environmental conditions that are difficult to anticipate during the development phase. 

Finally, we plan to make our framework available as \textit{testing-as-a-Service} in order to collect and analyze high fidelity simulation testing requirements from UAV developers to continuously improve the applicability of \REALSIM.  

% \jch{Bring your test plan forward here from the conclusion}.





==> dronology.tex <==
\subsubsection{Dronology}
The Dronology system uses a centralized architecutre with sUAS operating the Ardupilot stack.
\jch{If we include dronology we will describe it briefly here i.e., Ardupilot. Centrally controlled.}

==> listings/config_all.tex <==
\def\caplb{JSON Snippet for enabling and configure \DW monitors}

\colorlet{punct}{red!60!black}
\definecolor{background}{HTML}{ffffff}
\definecolor{delim}{RGB}{20,105,176}
\colorlet{numb}{magenta!60!black}





\lstdefinelanguage{json}{
    % basicstyle=\normalfont\ttfamily,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    numberstyle=\scriptsize,
    stepnumber=1,
    numbersep=8pt,
    showstringspaces=false,
    breaklines=true,
    frame=lines,
    backgroundcolor=\color{background},
    literate=
     *{0}{{{\color{numb}0}}}{1}
      {1}{{{\color{numb}1}}}{1}
      {2}{{{\color{numb}2}}}{1}
      {3}{{{\color{numb}3}}}{1}
      {4}{{{\color{numb}4}}}{1}
      {5}{{{\color{numb}5}}}{1}
      {6}{{{\color{numb}6}}}{1}
      {7}{{{\color{numb}7}}}{1}
      {8}{{{\color{numb}8}}}{1}
      {9}{{{\color{numb}9}}}{1}
      {:}{{{\color{punct}{:}}}}{1}
      {,}{{{\color{punct}{,}}}}{1}
      {\{}{{{\color{delim}{\{}}}}{1}
      {\}}{{{\color{delim}{\}}}}}{1}
      {[}{{{\color{delim}{[}}}}{1}
      {]}{{{\color{delim}{]}}}}{1},
}

\noindent\begin{minipage}{\textwidth}
\lstset{basicstyle=\tiny,style=jsonlistingstyle,  caption=\caplb, label=lst:test_scenario_config, xleftmargin=5mm,framexleftmargin=5mm,
    string=[s]{"}{"},
    stringstyle=\color{black}, %%% should only highlight value strins (but does not work atmm....}
   comment=[s]{:"}{"}
    commentstyle=\color{black},
}

\begin{lstlisting}
{
	"Drones": [{
		"VehicleType": "PX4Multitotor",
		"X": 0,"Y": 0,"Z": 0,
    "Pitch": 0,"Roll": 0,"Yaw": 0,
		"Sensors": {
			"Barometer":{"Type": 1,"UpdateFreq": 50},
			"Magnetometer":{"Type": 4,"UpdateFreq": 50},
			"GPS":{"Type": 3,"UpdateFreq": 50}},
		, {
        "VehicleType": "PX4Multitotor",
        ...}],
	"Environment": {
		"Wind": {
			"Direction": "NE","Velocity": 1},
		"Origin": {
			"Name": "Michigan Lake Beach",
			"Latitude": 42.211223,
			"Longitude": -86.390394,
			"Height": 164
		},
		"TimeOfDay": "08:00:00"
	},
	"Monitors": {
		"min_sep_dist_monitor": {
			"param": [
				"10"
			]}
	}
}
\end{lstlisting}
\end{minipage}
\vspace{-12pt}






==> listings/env_config.tex <==
\colorlet{punct}{red!60!black}
\definecolor{background}{HTML}{ffffff}
\definecolor{delim}{RGB}{20,105,176}
\colorlet{numb}{magenta!60!black}

\lstdefinelanguage{json}{
    % basicstyle=\normalfont\ttfamily,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    numberstyle=\scriptsize,
    stepnumber=1,
    numbersep=8pt,
    showstringspaces=false,
    breaklines=true,
    frame=lines,
    backgroundcolor=\color{background},
    literate=
     *{0}{{{\color{numb}0}}}{1}
      {1}{{{\color{numb}1}}}{1}
      {2}{{{\color{numb}2}}}{1}
      {3}{{{\color{numb}3}}}{1}
      {4}{{{\color{numb}4}}}{1}
      {5}{{{\color{numb}5}}}{1}
      {6}{{{\color{numb}6}}}{1}
      {7}{{{\color{numb}7}}}{1}
      {8}{{{\color{numb}8}}}{1}
      {9}{{{\color{numb}9}}}{1}
      {:}{{{\color{punct}{:}}}}{1}
      {,}{{{\color{punct}{,}}}}{1}
      {\{}{{{\color{delim}{\{}}}}{1}
      {\}}{{{\color{delim}{\}}}}}{1}
      {[}{{{\color{delim}{[}}}}{1}
      {]}{{{\color{delim}{]}}}}{1},
}


\def\capla{JSON Snippet for configuring the simulation environment. In this example\, two sUAS (denoted as sUAS1 and sUAS2) are configured to conduct a river search-and-rescue mission in windy conditions and bright lighting conditions}

\noindent\begin{minipage}{\textwidth}
\lstset{style=jsonlistingstyle,  caption=\capla, label=lst:env_conf, xleftmargin=5mm,framexleftmargin=5mm,
    string=[s]{"}{"},
    stringstyle=\color{black}, %%% should only highlight value strins (but does not work atmm....}
   comment=[s]{:"}{"}
    commentstyle=\color{black},
}
\begin{lstlisting}
{"Vehicles": {
    "sUAS1": {
      "VehicleType" : "PX4Multirotor",
      "UseTcp": true,
      "Sensors": {...}
    },
    "sUAS2": {...}
  },
  "OriginGeopoint": {"lat": 7.322,"long": 0.16273,  "alt": 122},
  "Wind": { "N": 10, "E": 1, "D": 2 },
  "Lighting": {
    "Enabled": true,
    "Time-of-day": "Morning",
    "Intensity": "Bright"
  },
  "Scene": {
    "TerrainType": "River",
    "Person": [
      {
        "id": "vic_0034",
        "Geo_loc": {"lat": 7.393,"long": 0.219 }
      }
   ]},
  "Real Geographic site": "XXXXX"}
\end{lstlisting}
\end{minipage}
\vspace{-12pt}

==> listings/test_props.tex <==
\def\caplb{JSON Snippet for enabling and configure \DW monitors}

\colorlet{punct}{red!60!black}
\definecolor{background}{HTML}{ffffff}
\definecolor{delim}{RGB}{20,105,176}
\colorlet{numb}{magenta!60!black}





\lstdefinelanguage{json}{
    % basicstyle=\normalfont\ttfamily,
    basicstyle=\footnotesize\ttfamily,
    numbers=left,
    numberstyle=\scriptsize,
    stepnumber=1,
    numbersep=8pt,
    showstringspaces=false,
    breaklines=true,
    frame=lines,
    backgroundcolor=\color{background},
    literate=
     *{0}{{{\color{numb}0}}}{1}
      {1}{{{\color{numb}1}}}{1}
      {2}{{{\color{numb}2}}}{1}
      {3}{{{\color{numb}3}}}{1}
      {4}{{{\color{numb}4}}}{1}
      {5}{{{\color{numb}5}}}{1}
      {6}{{{\color{numb}6}}}{1}
      {7}{{{\color{numb}7}}}{1}
      {8}{{{\color{numb}8}}}{1}
      {9}{{{\color{numb}9}}}{1}
      {:}{{{\color{punct}{:}}}}{1}
      {,}{{{\color{punct}{,}}}}{1}
      {\{}{{{\color{delim}{\{}}}}{1}
      {\}}{{{\color{delim}{\}}}}}{1}
      {[}{{{\color{delim}{[}}}}{1}
      {]}{{{\color{delim}{]}}}}{1},
}

\noindent\begin{minipage}{\textwidth}
\lstset{basicstyle=\tiny,style=jsonlistingstyle,  caption=\caplb, label=lst:monitor_config, xleftmargin=5mm,framexleftmargin=5mm,
    string=[s]{"}{"},
    stringstyle=\color{black}, %%% should only highlight value strins (but does not work atmm....}
   comment=[s]{:"}{"}
    commentstyle=\color{black},
}

\begin{lstlisting}
{"Properties": [
  { "Horizontal-Sep-Distance": {
    "Enabled": true,
    "Config": {
    "Min_sep": 10 },
      "Params": {
        "UAV": [ "ID", "Pos", "Dist" ]}}},
  {"Lateral-Sep-Distance": {
    "Enabled": true,
    "Config": {
    "Min_sep": 5 },
    "Params": {
      "UAV": [ "ID", "pos", "dist" ]}}},
  {"Collision": {
    "Enabled": true,
    "Params": {
      "Environment": ["o_ID", "o_name" ],
      "UAV": [ "ID", "pos", "impact_pos" ]}}},
  {"Human_Interaction": {
    "Enabled": true,
    "Config": {
      "Input_Source": "RC" }}},
  {"AI_Model_CV": {
    "Enabled": true,
    "Config": {
      "Target_id": "v_004" },
    "Params": {
      "Environment": [ "t_id", "t_pos" ],
      "UAV": ["detection_count","pos"]}}}]}
\end{lstlisting}
\end{minipage}
\vspace{-12pt}

==> old-configuration.tex <==
\section{Test Specification in \DW}
%System Tests Under Realistic Environmental Conditions}
\label{sec:specification}

Based on our analysis of sUAS safety literature and reported incidents we have collected that lead to the five basic requirements for an effective testing environment we have created our \DW architecture (cf.~\citesec{drarchitecture}) and an accompanying process for creating and  specifying mission-specific test configurations.
In the following, we briefly introduce our \DW test creation process and the capabilities provided by the framework. 
In order to accommodate both, the characteristics of the sUAS system under test, as well as the mission-specific characteristics that need to be taken into account we have decided to split a DW Test Specification into two main parts (A) the actual \emph{Test Case} and (B) a corresponding \emph{Test Scenario} that together serve as an input for a Testrun in the \DW testing environment. 
Test cases specified for execution in \DW include {\it configuration parameters} describing the real-world environment in which the test will be executed, a set of properties to be monitored and validated, and the executable sUAS `missions'.

For example, the following test specification provides a description of the test, defines specific environmental conditions that are configurable within the simulation space, lists safety properties, and describes expectations of the mission that the user is expected to deploy for the test. In practice, many safety properties are ubiquitous to each and every test cases, whilst others are mission-specific. The two sections of the test case labeled \emph{configuration parameters} and \emph{monitorable safety properties} specify how the environment will be setup and how objects (specifically sUAS) flown in the environment will be monitored. However, the final section labeled \emph{Test Flight} loosely describes the externally defined mission that will be deployed. This is interchangeable, as the platform user could execute many different missions in the same environment with goals of testing different types of behavior.  
\input{tables/tab_example_test}








\mv{Also I would describe these things more from a ``what is required for a good validation framework''.
(1) we need to configure the environment (and vary env. properties during simulation $==>$ Weather and Lighting Factors)
(2) There needs to be a proper environment - especially when you are flying certain type of misisons - e.g. finding a missing hiker, performing simulations in an empty are does not make sense, or when flying close to a river, etc... $==>$  Real World Location and in turn (3)  Mission Specific Scenarios for a particular purpose (e.g. river resuce/surveilance different things need to be tested, collected...
(4) data monitoring (i.e. a way to collect data from the simulator and real workd and compare/collect/analyze them - > hence the digital Twin (btw. we need to be a bit careful what we actually call a digital twin.
The thing we have now is more a ``Digitial Shadow'' rather than a twin - as a Twin per definition has the ability for bi-directional data  exchange (i.e. collect data from the sytem, run simulations and send data back to the drone to improve/update something).}






% \subsection{Configuration Parameters}
% sUAS are particularly sensitive to their environments and therefore it is important to test them within context. As illustrated in our example, configurable parameters include weather, location, scene, and signal attributes. 


% \bulletitem{Weather and Lighting Factors} such as wind, fog, rain, and specific lighting conditions (sunny, dawn, dark),  greatly impact the functioning of both the UAV's perception of the environment and its control algorithms \cite{gao2021weather}, and thereby affect system safety. Wind speed is often cited as a cause of UAV crashes because high wind speed  in a particular direction can negatively affect the ability of the UAV to maintain its desired flight path \cite{lundby2019towards}. Furthermore, rain, fog, and snow, as well as low lighting conditions in the environment, impair the ability of computer vision models to interpret the environment correctly \cite{hamzeh2022improving}. Further, GPS signal quality continuously varies in the real world impacting autonomous navigation and autonomy computations, as discussed in \cite{Ankit's paper}. Therefore, \DW supports configuration and simulation of various weather conditions, and position of the sun (i.e., time of day) which creates various shades of lighting conditions.
% \input{tables/tab_weather}

% \bulletitem{Realistic Location settings}
% Standard UAV simulators such as Gazebo \cite{koenig2004design} include an empty environment or simple three-dimensional shapes such as cylinders and cubes as obstacles for UAVs to avoid. These simulation environments fail to capture the complexity of the shapes, sizes, textures, and terrains found in the real world. High-fidelity simulation environments that support rigorous integration and acceptance tests, need to incorporate real world environmental data.  This would allow test cases to validate whether a UAV can operate safely by avoiding trees or tall buildings, and whether it can plan routes that do not violate societal boundaries and impact individual privacy. Table \ref{tab:geo_props} shows examples of properties that can be configured into a simulated environment. These include the selection of digital twins of cities, safe landing stations within cities, restricted airspaces within the  cities for UAVs to avoid, and various  objects such as birds, pylons, and other flying vehicles. 
% \jch{Needs to be a bit more substantiated with references from other simulation environments etc. We can also reference our own use cases (in 3rd person)}.
% \input{tables/tab_realworld}

% \bulletitem{Mission Specific Scenarios} The inclusion of custom landscapes and environments to support acceptance tests associated with realistic real-world scenarios is essential for testing the run-time behavior of the system as a whole. For example, the simulated environment for a UAV-supported river search and rescue operation could include a river, and an animation of a person struggling in the water with intermittently visible parts of their body as they move up the water level for a short amount of time before temporarily submerging. A simulation environment of this nature would test the effectiveness of integrating control algorithms, such as tracking or following the victim, with perception algorithms, such as detecting the victim.  Since designing such complex mission specific scenarios requires huge effort and time of UAV software developers, we aim to add landscapes and dynamic objects in support of extensive real-world scenarios into our simulation environment. UAV software developers will select scenarios and configure their properties to create customized simulations. Table \ref{tab:scenario_props} shows a subset of potential configurable properties for river search-and-rescue and fire surveillance missions. 
% \input{tables/tab_scene}

% \bulletitem{Signal and Interference}
% \jch{@Ankit -- I think we can reference your (hopefully) new paper to talk about signal and HDOP. Also there was a talk at the Aviation/NASA conference about GPS loss behind buildings etc so I think we can set the scene here.} This section talks about wireless availability, interference, satellites (RTK option?), n3 (??) etc. the noise inherent to radio signal strength, and variations in GPS satellite count availability as summarized in Table \ref{tab:interference_feature}.
% \input{tables/tab_signal}

% \bulletitem{Human Interaction}
% \jch{Something about human interactivity. I'm thinking (as per original test case example) that we might start simple and allow interactivity via RC and/or stream monitored data for the user application to use.)  Note: in our current deployment we already have some 'dangerous' human interactions, so we could mention these.  We crashed one drone based on this.}
% \input{tables/tab_humans}


% \subsection{Monitorable Properties}
% \mv{what needs to be monitored and why?}

% We leveraged three different sources of information to identify a set of sUAS-related safety properties which we monitor by default unless explicitly turned off by the user or irrelevant to the specific context. Several examples are shown in Table \ref{tab:example_spec}.

% Our data sources included (1) a Systematic Literature Review (ask MV about the ones we ignored for our HIP FSE student because they weren't human related), (2) the section in sUAS documentation manuals describing emergency procedures as define a set of unwanted cases which need to be monitored for, with (3) the final list of properties augmented from our own domain knowledge of sUAS flying. 

% Something about how users can augment properties.


















% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=.8\textwidth]{./figures/approach_realfightSim.pdf}
%     \caption[Simulation Testing Approach in \REALSIM]{Simulation Testing Approach in \REALSIM. \textit{F1}, \textit{F2}, and \textit{F3} represents three different features of the environment. P1, P2, and P3 represents three specific properties of the system under test. \jch{@Ankit (1) I think we need to have another box in the top left representing a tester's independent sUAS application that they bring to the test platform.  This is referenced by the test scenario, but then accesses the Configured Realistic Environment via a well-defined API. So we probably want to depict the API too. (2) Can you lighten the gray color so it prints a little better.  Maybe we could use a different color for the external sUAS application too, and (3) I think we need to have two different boxes for "Test Scenario" and "Test Case".  The system properties feed into Test Case (not Scenario). Splitting in this way will allow us to incorporate a bit more of the requirements into the paper, and I think this will make a stronger ICSE paper (and stronger NASA proposal too).}}
%     \label{fig:realflightsim_approach}
% \end{figure*}














% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\columnwidth]{./figures/ENVFramework.drawio.png}
%     \caption{Overview of Categories in which  Environmental Properties and System Properties must be specified in order to design and generate  acceptance test artifacts. }
%     \label{fig:test_rules}
% \end{figure}
% Typo on "Environment PropOERties" \jch{Ankit I think the Flight and HoTL ones still need work. See this document: \url{https://docs.google.com/document/d/12WgCNnz_xCZ3HKj3Gcs03yKtEgv4PmivxT9E86plZXw/edit?usp=sharing}}

%\section{Monitorable System Properties}

\subsection{Runtime Monitoring}
How do we define them, monitor for them etc etc.


\subsection{Results Generation and Analysis}
UAV software consists of run-time monitoring programs for continuously observing and analyzing run-time behavior, including vehicle parameters, mission parameters, and autonomy model parameters. While we expect users of \REALSIM (e.g., Droneresponse developers) to independently monitor the runtime behavior of their own UAVs, we also plan to monitor this behavior directly in \REALSIM. Further, \REALSIM also monitors properties of the simulated environment to ensure that the simulation environment matches the specified test conditions, and to detect UAV interactions with the environment such as collisions with buildings, trees, or other UAVs. During the execution of each configured simulation, applicable system properties are monitored using  the monitoring capabilities of the UAV system and the simulation environment. If any  properties are violated then the violations are displayed and the test fails. The data collected from both the system monitors and the environment monitors can be synchronized by timestamps to automatically generate a simulation report that provides insight into the run-time behavior of the system to perform test diagnosis.

% \jch{The following needs replacing based on what we find from the above study.   }
% We also define a set of system properties specifying functional, safety, fairness, and usability qualities. Some system properties are expected to hold true across all acceptance tests, while others are applicable to specific tests.  As shown in  Figure \ref{fig:test_rules} we classify system properties into three primary categories of \emph{Mission} properties, \emph{HoTL}, and \emph{Perception} properties. 

% \subsection{Mission Properties}
% Mission properties are typically defined in terms of sensor data (e.g., GPS, gyroscopes, accelerometers, and magnetometers) which is indicative of UAV health throughout the mission, general mission information (e.g., separation distance between UAVs, ability to reach a safe landing station, authorized airspace, traversal of target waypoints), and control algorithms \cite{nguyen2020control} that define the run-time behavior of UAVs during a mission. 
% %Failure to acquire high-quality sensor data, communicate with other UAVs or software-based Ground Control Stations where  mission failure and compromise system safety. 
% Therefore, we have incorporated the following properties into our framework to support tests in different environmental configurations. 

% \noindent {\it S1: Flight:}
% In order to test the ability of the system to fly safely under a variety of environmental conditions, a complete mission is assigned to one or more UAVs. Tests based on flight properties validate whether UAVs in the mission are able to complete their assigned flight path under available resources such as battery, and whether they self-adapt their flight path as needed to complete the mission. \new{For example, in the \REALSIM environment, CPS developers could configure extreme windy conditions to test a UAV's capability to complete a mission. The run-time monitoring of battery voltage, vibration, and velocity would provide insights regarding a UAV's ability to fly successfully in real-world windy conditions.}

% \noindent {\it S2: Collision Avoidance:}
% \new{CPS developers impose multiple constraints on dynamically generated flight plans as well as UAV maneuvers to avoid collisions with} trees or buildings, other unmanned vehicles, and birds etc. Collision avoidance properties test whether the system constraints are sufficient to prevent collisions with objects in the environment, including other UAVs in the mission. \new{An example of a safety constraint for avoiding collisions is enforcing UAVs to maintain a minimum separation distance from other UAVs or objects in the environment. Test outcomes would enable developers or operators running preflight tests, to simulate a multi-UAV mission to verify whether the configured minimum separation distance is sufficient under extreme weather conditions, within a dense city environment, or in other specified operating environments. By monitoring run-time properties, such as the separation distance between the UAVs or the occurrence of actual collisions, would help validate the system design and support incremental improvements until tests passed consistently in anticipated operating conditions.}

% \noindent {\it S3: Restricted Airspace Avoidance:}
% During a mission, UAVs are prohibited from entering certain airspace in order to maintain air safety, as per FAA Guidelines. For instance, UAVs must avoid critical airspace such as class B airports and are prohibited from flying over landmarks such as stadiums, prisons, and hospitals. Furthermore, UAV operators typically create a safe geo-area in which UAVs are expected to remain in order to ensure mission safety. As a result, the Restricted Airspace Avoidance properties test whether the system is able to detect and avoid different restricted airspace in a variety of environmental conditions. For instance, developers could test whether a UAV is capable of avoiding restricted airspace when the GPS signal quality is very poor. Monitoring access to restricted airspace, UAV flight paths, and GPS signal quality would provide valuable insights into the system's ability to avoid restricted airspace in the real world.

% \subsection{HoTL Properties}
% Humans-on-the-Loop play a critical role in ensuring system safety, and humans and UAVs often need to collaborate on tasks together. Therefore, the HoTL properties of our framework specifically aim to test the Human-UAV interactions during an emergency response mission. These properties are derived from the primary goals of effective coordination and control between humans and machines namely  \textit{Transparency}, \textit{Augmented Cognition}, and \textit{Coordination} \cite{mcdermott2018human,cleland2022extending}. 

% \noindent {\it S4: Transparency:}
% As discussed in Chapter \ref{ch:chi2020}, situational awareness, defined at three different levels \cite{endsley2001designing} is crucial for effective Human-UAV partnerships. Further, in Chapter \ref{ch:autonomyExplanations}, we showed how \droneresponse provides necessary information in the form of explanations to keep humans aware of the situation. As a result, transparency properties, evaluated through user studies, test whether the system provides sufficient information about the environment and autonomous decision-making in various environmental conditions to keep humans sufficiently aware of the mission status.

% \noindent {\it S5: Augmented Cognition:}
% Automated UAVs are capable of adapting their plans, and requesting assistance from humans at different points in the mission in response to dynamic environmental changes. As discussed in Chapter \ref{ch:modre2020}, humans intervene into the UAV autonomy by providing \textit{feedback}, \textit{sharing knowledge} about the environment, and \textit{sending control commands}. These human interventions are generally intended to guide UAVs towards their mission objectives or to mitigate emergent hazards during the mission. The simulation environment enables user tests to validate whether the system provides users with capabilities and  opportunities to intervene in the autonomy of the UAVs when deemed necessary, under a variety of environmental conditions.

% \noindent {\it S6: Coordination:}
% During a mission, humans may acquire full manual control of an autonomous UAV to accomplish a task for a variety of factors such as the trustworthiness and reliability of the UAV in a specific mission scenario. Thus, the system relinquishes control of the mission to human users, and later, after obtaining permissions from humans, regains control. This notion of permission based autonomy control is discussed in Chapter \ref{ch:modre2020}). These properties are therefore designed to test the seamless transition of control between humans and UAVs during an emergency response.                                                                      

% \subsection{Perception Properties}

% Autonomous UAVs build their awareness of the environment using computer vision models  such as YOLO \cite{yolo_redmon2016you}. Failure to correctly recognize different elements of the environment cause UAVs' to behave unpredictably. Perception properties aim to test whether a UAV is capable of perceiving the environment correctly in various environmental conditions. 

% \noindent {\it S7: Confidence:}
%  As discussed earlier, the performance of a computer vision (CV) model is verified using images in the validation datasets, which may not represent all complexities of the environment. The differences between the validation datasets and real environmental conditions affect UAVs' perception, resulting in the system failure. In particular, the confidence metric of a model indicates the probability that it has recognized an element such as person, or birds in the environment correctly \cite{pouget2016confidence}. As a result, we included this property in our framework to test whether the computer vision model is capable of producing sufficient confidence under challenging environmental conditions or when used in multi-UAV scenarios in which UAVs may need to collaboratively agree and act upon their perceptions. Evaluating the use of CV models within simulation environments highlights the need for high-fidelity imagery.
 
% \noindent \textit{S8: Bias:}
% Computer vision models may be subject to bias due to their programming and data sources. As an example, a model may classify any person in the river as a drowning person. However, this is not always the case, as the UAV may have captured a person who was swimming in the river. The lack of swimmers in the data set on which the computer vision model is trained results in an inaccurate perception of the UAV. As a result, we included this property in our framework to test whether the UAV's perception is free from any possible bias or not. 


% % \jch{Ankit - maybe mention in 1-2 sentences that each system property is supported by one or more reusable test. For example, a system property stating that ``Minimum separation distance (MSD) must be maintained between all UAVs throughout the flight'' is supported by a dynamic test case that monitors distance between UAVs and fails when MSD is violated.}


% \section{Simulation Test Cases}

% \subsection{Test Case Specification}
% Given the available set of system properties and the configurable simulation environment, a developer (or dedicated tester) specifies an integration or acceptance test. The test includes three components: (1) a description of the mission or tasks to be performed by one or more UAVs, (2) a description of the simulation environment in which the mission is to be executed, and (3) a set of system properties that are expected to hold during the mission. Once the test case is written, the tester configures the simulation environment using the simulation configuration properties, defines a specific mission to be performed by one or more UAVs, and executes the test case by launching the mission and monitoring for any violations of system properties. We provide concrete examples of two tests that could be run in simulation to validate specific properties, in order to generate evidence of the system's safety. These tests align with the system properties shown in Figure \ref{fig:test_rules}.


% \begin{table}[htbp]
% \small
%     \centering
%     \caption{Simulating two different configurations of Environmental Features}
%     \label{tab:river_config}
%     \begin{tabular}{|c|c|c|}
%     \hline
%     \textbf{Environment Features}&\textbf{Configuration 1 (C1)}&\textbf{Configuration 2 (C2)} \\ \hline
% Environmental Factors&Wind = 23 mph & Rain = Heavy \\ \cline{2-3}
% & Time of Day = Afternoon&Time of Day = Evening \\ \hline
% Mission Specific Scen. &S= S\&R &S= S\&R \\ \cline{2-3}
% &River W= 10m, V=3mph, D=West& --- \\ \cline{2-3}
% &Victim A=20, G = M, H=5'10''&Victim A=50, G=F, H=5'10'' \\ \cline{2-3}
% &visible body part = Lower body&Visible body part = hands \\ \hline
% Geographic Sites&---&Region = Saint Joseph River \\ \hline
%     \end{tabular}
    
% \end{table}


% \begin{table}[htbp]
% \small
%     \centering
%      \caption{System Properties Under Test for two different environmental Configurations in the simulated Environment}
%     \label{tab:sys_props_river}
%     \begin{tabular}{|c|c|p{7cm}|c|}
%     \hline
%          \textbf{S. No} &\textbf{System Property}&{\multicolumn{1}{c}{\textbf{Example of a test}}} &\textbf{Env Config} \\ \hline
% S1&Flight & UAV battery never goes below 10\% during flight&C1, C2 \\ \hline
% S2&Collision Avoidance& UAV avoids collision with trees&C2\\ \hline
% S3&Airspace Avoidance& UAVs never enters any restricted airspace of a city&C2\\ \hline
% S4&Transparency& UAVs provide humans with sufficient and accurate explanations about mission status & C1, C2\\ \hline
% S5&Augmented Cognition& When UAVs track an object that is not a victim, human intervention to manually control the UAV is always successful & C1, C2\\ \hline
% S6&Coordination&UAVs avoid tracking objects that look like victims if they have previously been identified as “not victims” by a human operator. &C1, C2\\ \hline
% S7&Confidence& UAVs are capable of detecting a drowning individual in a river with a high degree of confidence (above 80 percent)&C1, C2\\ \hline
% S8&Bias& UAV is capable of detecting victims in the river regardless of their gender and visible body parts&C1, C2 \\ \hline
%     \end{tabular}
   
% \end{table}

% Each example shows a distinct configuration of the simulated environment. For example, configuration 2 (C2) represents the environmental conditions with the contextual information of: \textit{During heavy rain, around 5 PM at a section of the Saint Joseph River, a 50-year-old female of height 5'10'' has drowned and only her hands are visible.} Table \ref{tab:river_config} shows how each example is configured by setting simulation configuration properties in the simulator.



%  Table \ref{tab:sys_props_river} shows an example test for each system property in one or more environmental configurations. In practice, we would define a suite of tests for each type of property. For instance, S7 in Table \ref{tab:sys_props_river} examines whether a UAV can accurately detect a drowning person in both rainy and windy conditions. Similarly, S8 examines whether the UAV's computer vision model is biased against recognizing drowning victims of particular genders or not. Depending on the configuration of the environment, relevant properties of the system are chosen for testing. For instance, in Environmental Configuration C1 (Table \ref{tab:sys_props_river}), all properties are tested except for P3 (Restricted Airspace Avoidance) as the configured environment does not contain restricted airspace of a city, and P2 (under Collision Avoidance) since trees are not configured in the environment. All properties are tested for C2 (Table \ref{tab:river_config}), including P2 and P3, as the environment contains a region of a real city with trees.

%  \jch{Ankit: I think you need to just say, that you then plan an actual mission with UAVs, then all ubiquitous tests are activated, and mission-specific ones activated when relevant.  For example, in your table, tests associated with system properties 1, 4, 5, 6, 7, 8 are relevant to both tests, but S2 and S3 is only relevant to C2.  Actually, I would think 2 and 3 are also relevant to ALL.  If you have a single UAV example, and you have a property about UAV to UAV collisions, then that would be an example of a property that only activates under certain conditions.}

% As explained above, each of these proposed acceptance tests is supported by a suite of lower-level tests that check whether the relevant system properties hold throughout the test.



% \jch{MAJOR COMMENT HERE:  What yo need is a section on system properties with examples that map to the categories in Figure 1.1.  This should be separate from the scenarios.  In other words you need a section (which you have) that discussed the Simulation Configuration Properties, now you need a separate section on System properties, and FINALLY, you need a section that shows how both of these come together for specific scenarios.  You are missing the 'clean' and 'distinct' section on System properties (see the google sheet).}





% \begin{table}[htbp]
%     \centering
%     \caption{Configuration of Environmental Features to conduct simulation test for river search-and-rescue scenario}
%     \label{tab:river_env_config}
%     \begin{tabular}{|c|c|}
%     \hline
%          \textbf{Environment Features}	& \textbf{Configuration}  \\ \hline
%         \multirow{2}{*}{Environmental Factors}	& Wind=23 mph \\ \cline{2-2}
% 	& Time of Day = Afternoon \\ \cline{2-2}
% 	& GPS signal Quality = Good \\ \hline
% \multirow{4}{*}{Scenario Specific Component}& Scenarios = River Search and Rescue \\ \cline{2-2}
% 	& River Width = 10 m, Velocity=3mph, Direction=West \\ \cline{2-2}
% 	& Victim Age = 20, Gender = Male, Height=5'10'' \\ \cline{2-2}
% 	& Visible body part = Lower body \\ \hline
%     \end{tabular}
    
% \end{table}














% \subsection{Mission Properties}

% UAVs can complete a mission within the available battery power in foggy and dark weather conditions (\emph{Environmental Factor})
% UAVs can plan a safe route to deliver flotation devices (\emph{Mission Specific Scenarios})
% \noindent \textbf{S1: Individual / Multiple UAV Mission: } 


% In the context of river search-and-rescue missions, the simulation should demonstrate that (a) UAVs can complete a mission within the available battery power in foggy and dark weather conditions (\emph{Environmental Factor}), (b) UAVs can plan a safe route to deliver flotation devices (\emph{Mission Specific Scenarios}), and furthermore that (c) autonomous UAVs are capable of executing the mission in a realistic geographical location such as in a section of the St. Joseph River (\emph{Real Geographic Sites}). 

% \noindent \textbf{S2: Collision Avoidance:}

% In the context of a crime-surveillance mission, a test case in simulation could demonstrate that (a) UAVs are capable of avoiding collisions and re-planning their routes in conditions such as fog, snow, and rain, which have a direct impact on the visibility of UAVs (\emph{Environmental Factor}), (b) UAVs are capable of tracking a car driven at high speed by a criminal (\emph{Mission Specific Scenarios}), and (c) UAVs are capable of avoiding collisions with buildings and trees in a realistic city such as Boston or where the system is intended to be deployed (\emph{Real Geographic Sites}).    

%  \noindent \textbf{S3: Restricted Airspace Avoidance:}
 
%  The simulation test should demonstrate that (a) the system is capable of avoiding restricted airspace even if the GPS signal strength is not excellent (\emph{Environmental Factor}), (b) the system can detect a dense crowd at run-time and avoid flying over it  (\emph{Mission Specific Scenarios}), (c) UAVs can fly through a real geographic area while avoiding all the restricted airspace within the city (\emph{Real Geographic Sites}). 


 
 
% %  \subsection{Human-on-the-Loop Properties:}
 
 
% %  \noindent \textbf{S?: Transparency:}

 
% %  Therefore, the simulation tests should demonstrate that the system provides sufficient information regarding (a) the environmental conditions in which the UAV is operating, (b) automatically generated plans to achieve a mission-specific task, and (c) the geographical area in which a UAV is operating by using specific street names and landmarks of a city in the reasoning. During simulation tests, a human observer should monitor the autonomous mission through a graphical user interface, including aerial video streams, and verify that the system is transparent and provides sufficient information to understand the status of the mission. 

% % \noindent \textbf{S?: Augmented Cognition:}


% % For a river search-and-rescue mission, the simulation must demonstrate that (a) a human observer can quickly comprehend the weather alert provided by the UI (\emph{Environmental Factor}), analyze the aerial video stream to identify possible human actions, and intervenes into the UAV autonomy for safety, (b) human intervention in critical scenarios such as victim tracking, or flotation device delivery does not impact the expected functioning of onboard autonomy models (\emph{Mission Specific Scenarios}), and (c) humans are able to safely intervene to rescue a person from a realistic geographic site (\emph{Real Geographic Sites}). 

% % \noindent \textbf{S?: Coordination:}

 
% %  For example, consider that the UAV perceives a rock in the river as a potential drowning victim and switches to Tracking Mode. However, the human observer denies the presence of a victim and commands the UAV to change to Searching Mode. In this case, the UAV switches to Searching Mode for a few seconds, but once again identifies that rock as a victim and switches back to Tracking Mode (\emph{Mission Specific Scenarios}). Such runtime behavior causes system instability, resulting in mission failure. Similar tests can be conducted for various Environmental Factors and real-world Geographical configurations of the environment. 
 

% % \noindent \textbf{S6: AI Confidence:}
 
 
% %  When a computer vision model is used to recognize different elements of the environment, such as people, trees, buildings, or birds, the simulation test (i) should verify the model's confidence under different weather conditions (\emph{Environmental Factor}) is above a certain threshold, (ii) demonstrate that the model detects drowning individuals in a river flowing at high velocity, where only the lower portion of the individual can be seen through the UAV's camera  (\emph{Mission Specific Scenarios}), and (iii) the model's performance in a realistic geographical site would provide insight into whether the model's unpredictability is acceptable to deploy in the real world or not (\emph{Real Geographic Sites}). 

% % \noindent \textbf{S7: AI Biases:}


==> old/Evaluation_old.tex <==
\section{Experimental Evaluation} 
\label{sec:sim_eval}
For our evaluation we derived three different research questions related to the efficacy of \DW for assessing and improving the robustness of an sUAS deployment in advance of a real-world deployment. We focused on this question primarily because of our own needs to deploy \DR safely in populated or otherwise potentially risky environments. For this reason our evaluation is qualitative in nature and uses our own real-world application scenarios as case studies. While these are non non-trivial in nature, and the evidence produced from the simulations was used in formal review documents by external agencies, we discuss associated limitations and threats to validity in Section \ref{sec:threats}. With our evaluation we address the following research questions \jch{Just a first attempt at these}.\\ 
\vspace{-3pt}

RESEARCH QUESTIONS HERE:
\begin{itemize}
    \item[RQ1:] Can we actually specify realistic test scenarios? (Matches Env. configuration and test scenario):  Address this through the use cases. (JSON as specification).
    \item[RQ2:] Original RQ1 -- can we detect problems and safety related issues?  
    Address this through running the simulation with some set of seeded "faults".  SEVERE WINDS. We can identify the point of failure. 
    %\item[RQ3:] Testing vignettes.  Can we demonstrate that what we see in the simulator matches what happens in the real world. (e.g., we map flight routes in the simulator against real-world).  
    \item 
\end{itemize}

\noindent\textbf{RQ1: To what extent does \DW~unearth problems and enable black-box validation of an sUAS system-under-test in realistic contexts prior to its deployment?} \\  We address this question by using \DW to generate test configurations for different real-world application scenarios and perform a series of test runs.
\vspace{6pt}

\jch{Somewhere claim that it works for PX4, Ardupilot, and a simple generic flight controller (??).}

% \noindent\textbf{RQ2: Does \DW~provide evidence that is useful for building a Safety Assurance Case? If so, what?} \\  %Honestly not sure about this, but we can see later.
% \vspace{-3pt}

%\noindent\textbf{RQ3: How flexible is \DW for easily adapting to different SuT and diverse deployment contexts?} \\  %Two different real-world deployments, two SuTs with entirely different architectures and different flight-controller stacks.

\\  To evaluate the last research question we applied \DW to a second SuT, with  different architectures, technologies and and different flight-controller stack, and captured the required effort to integrate the SuT in the \DW framework.

\vspace{-3pt} 

\subsection{Real-World Case Studies}

We evaluated \DW by using it to test our PX4-based system (\dr) for two real-world deployments, each of which had significant safety-concerns. However, before describing the use of \DW for these deployments we provide a brief overview of both systems under test (sUT). 


\input{drone-response}

\subsection*{Case \#1: Image Collection at Active Airbase (ImageCollect)}

For this use case, we deployed six Hexacopter sUAS using \DR at a test location on the grounds of an active airbase with air traffic in close vicinity. The purpose of this use case was to collect aerial imagery of people (hired actors) from diverse distances, pitches, and angles as part of a computer vision research project.
Prior to the deployment, both  hardware and control software had to undergo a rigorous safety review process and receive approval to operate under a Certificate of Authorization\footnote{More details will be provided after double blind review. For now, we upload the safety case we developed, including evidence obtained from use of the proposed simulation platform as supplemental material. This will be made publicly available when this work publishes.}. 

Data collection was centered around three adjacent locations (referred to as ``stations`'), with two sUAS assigned to each station. When in flight, each sUAS was tasked with executing a  designated flight pattern (different for each station), to  collect imagery at different altitudes, pitches, and distances. At each station, only one sUAS was allowed to fly at any time. The second sUAS was cleared for takeoff only after the first sUAS landed. Given the flight patterns of each sUAS, there was potential for overlap between the airspaces across the three stations. The airport authorities provided strict safety regulations, the majority of which were already covered by our default safety constraints; however,four additional constraints (labeled C1-C3) were added as mission-specific safety properties, and two (labeled C4-C5) as a critical property for achieving the non-functional requirement of acquiring clear images.  \jch{Formally define these using whatever language we decide to use.}
\begin{enumerate}
    \item[C1] Lateral distance must be maintained between all inflight sUAS at all times (i.e., an sUAS can never fly over another in-air sUAS). (Measurable property: Distance(D1(lat,lon),D2(lat,lon) ALWAYS > 20 meters) for each pair of drones in the air.)
   % \item[CX] \st{At each station, only one sUAS can be in the air at any time.} 
    \item[C2] The sUAS must not fly over no-fly zones including active taxiways or runways or areas designated as `actor' zones.
    \item[C3] The camera should never face into the sun.
   % \item[CX] \st{At least 10 seconds of imagery is collected with the actor within the center part of the screen for each targeted sUAS position. (Yolo identifies image within center 50\% of screen).}
    \item[C4] Abort takeoff due to sudden appearance of lots of big fat geese flying low over the launch pad.
\end{enumerate}

Based on the deployment scenarios, we imported a map of the airport associated with the region in which we would deploys the sUAS. As the map did not provide full 3D coverage of the relatively remote area, we added additional objects representing tall trees and a construction lift (used for raised cameras). Based on the use-cases of our planned deployment (as summarized above), we then specified the operating context as depicted in Table \ref{tab:briar-test}. 
\input{tables/tab_BRIAR_test}

To support fuzz testing that covers values within anticipated ranges of values we specify several properties as ranges allowing \DR to run multiple simulations that provide diverse coverage of the overall context space. For each simulation, \DW monitored the specified constraints, and output a report showing any violations.  
Exploring optimal strategies for covering this space is out of context of this paper, and therefore our experiments involved a heuristic approach. First, we executed every range at its high and low levels with all other ranged values (i.e., with five parameters defined as ranges) we have $5^2=32$ permutations. For any failed cases, we systematically performed a one-hop analysis by reducing each variable in turn to its other levels (i.e., high, medium, or low) to systematically explore the space. For each failure case (if any), this introduced an additional $5\times2$ simulations. 






% FIX THIS We evaluated the extent to which the set of available \DW properties provided coverage of our safety claims in the SAC, and where necessary specified additional safety constraints based on the monitorable data.  Based on this analysis we specified the test environment as shown in \jch{Something like TABLE 1 but for Griffiss/BRIAR}. Many of the safety properties of interest were already included in the default set of properties. For example.... However there was one additional  

\subsection*{Case \#2: Emergency Response Demo of Missing Child Search (WaterRescue)~} 
Our second case study deployed four six Hexacopter sUAS in support of a live search-and-rescue demonstration at a beach area in collaboration with emergency responders and lifeguards (Should be able to include PICS!). While there were no external safety assessors, the public nature of the demonstration, and the fact that it was conducted during the summer time  at a crowded beach area, led us to construct a safety case and perform rigorous testing before deployment. The demo enacted the scenario in which a report was received of a missing child, potentially swept out into the water. The sUAS were assigned a search area and dispatched to search, utilizing onboard computer vision, and to stream video when a potential sighting was made. In particular, we wanted to simulate the exercise in advance, to evaluate the impact of windy conditions coming off the water, and to ensure that the following critical safety properties held throughout the mission. In this case, all three were considered safety related, with two [C1, C2] directly related to flight safety, and one [C3] related to avoiding informational overload which is considered a situational awareness demon (REF).

\begin{itemize}
    \item[C1] No search flights will be conducted over the beach (given that it is highly populated with beach goers).
    \item[C2] No sUAS will land in the water. If urgent landing is needed, the sUAS will land at designated (supervised) point). 
    %\item[C3] \st{When multiple sUAS sight the same person, the data will be merged into a single user alert.}
    \item[C3] sUAS will not collide during emergency takeoffs.
    \item[C4] Routes to be within some degree of accuracy in VERY VERY VERY WINDY WEATHER. (Routes to be successful).
\end{itemize}

As with Case\#1, we specified these mission critical properties and environmental factors for configuring the simulator.  In this case, we limited the variations in favor of running a far larger number of test cases with different routing scenarios provided by the SuT. Furthermore, by setting up the simulation in this way, we were able to quickly rerun it in the final days with the forecasted weather conditions. The values in Table \ref{tab:mc-test} represent the actual environmental conditions of the field deployment.

\input{tables/tab_MC_test}.


\subsection{Validation Process}
For each of the use cases we followed the following process of exploring the different scenarios, designing the tests, specifying the test set up, executing the simulations and finally, analysing the results.  


Just mapping out a plan here...
\begin{enumerate}
    \item Explore scenarios (to make this more about 'requirements' and avoid the 'testing' reviewers I think we should provide actual use case scenarios)
    \item Design test contexts with some variability (fuzzing??) so that we can run mutants
    \item Add mission-specific properties as needed to the default ones.
    \item Design missions for each scenario (e.g., flight routes, coordination handlers etc etc)
    \item Execute simulation and check for violations of safety constraints.
\end{enumerate}

Something about running STRESS tests in the simulator and real tests under 'normal conditions in the real world.

But we also need to demonstrate some results.  We could show how these results served as evidence in the safety case that was acceptable to nuair (Griffiss). We could collect some numbers.

% \subsection{RQ3: Application}
% \subsection{RQ1: Validation Tests}
% \subsection{RQ2:Safety Assessment}

\subsection{Fidelity Testing}
Short section on fidelity testing. 



==> old/configuration_backup.tex <==
\section{Test Specification in \DW}
%System Tests Under Realistic Environmental Conditions}
\label{sec:env_framework}


\begin{figure*}[t]
    \centering
    \includegraphics[width=.8\textwidth]{./figures/approach_realfightSim.pdf}
    \caption[Simulation Testing Approach in \REALSIM]{Simulation Testing Approach in \REALSIM. \textit{F1}, \textit{F2}, and \textit{F3} represents three different features of the environment. P1, P2, and P3 represents three specific properties of the system under test. \jch{@Ankit (1) I think we need to have another box in the top left representing a tester's independent sUAS application that they bring to the test platform.  This is referenced by the test scenario, but then accesses the Configured Realistic Environment via a well-defined API. So we probably want to depict the API too. (2) Can you lighten the gray color so it prints a little better.  Maybe we could use a different color for the external sUAS application too, and (3) I think we need to have two different boxes for "Test Scenario" and "Test Case".  The system properties feed into Test Case (not Scenario). Splitting in this way will allow us to incorporate a bit more of the requirements into the paper, and I think this will make a stronger ICSE paper (and stronger NASA proposal too).}}
    \label{fig:realflightsim_approach}
\end{figure*}







\jch{I think this section needs to focus almost entirely on how we define tests.}
\mv{I think this starts way too \DW specific - What is probably required is some general introduction on how these kind of tests work - what is required, etc. 
if we  go with the DigitalTwin buzzword we probably need to talk about test cases, building a digital representation for validation as well as hardware in the loop testing - which then combines simulation + real workd testing, resulting in a holistic test environment.

$===>$ https://ieeexplore.ieee.org/abstract/document/9213676/
}
\jch{Is digital "shadow" a thing?  I like it anyway, but did you make it up or is it a thing?  Either way we should use that term!}

\mv{Also I would describe these things more from a ``what is required for a good validation framework''.
(1) we need to configure the environment (and vary env. properties during simulation $==>$ Weather and Lighting Factors)
(2) There needs to be a proper environment - especially when you are flying certain type of misisons - e.g. finding a missing hiker, performing simulations in an empty are does not make sense, or when flying close to a river, etc... $==>$  Real World Location and in turn (3)  Mission Specific Scenarios for a particular purpose (e.g. river resuce/surveilance different things need to be tested, collected...
(4) data monitoring (i.e. a way to collect data from the simulator and real workd and compare/collect/analyze them - > hence the digital Twin (btw. we need to be a bit careful what we actually call a digital twin.
The thing we have now is more a ``Digitial Shadow'' rather than a twin - as a Twin per definition has the ability for bi-directional data  exchange (i.e. collect data from the sytem, run simulations and send data back to the drone to improve/update something).}


\mv{Ideally, all these requirements then guided the development of \DW }
\mv{I would say, all the tables and properties are already a concrete contribution and I would describe them separately afterwards}




Test cases specified for execution in \DW include {\it configuration parameters} describing the realworld environment in which the test will be executed, a set of properties to be monitored and validated, and the executable sUAS `missions'. For example, the following test specification provides a description of the test, defines specific environmental conditions that are configurable within the simulation space, lists safety properties, and describes expectations of the mission that the user is expected to deploy for the test. In practice, many safety properties are ubiquitous to each and every test cases, whilst others are mission-specific. The two sections of the test case labeled \emph{configuration parameters} and \emph{monitorable safety properties} specify how the environment will be setup and how objects (specifically sUAS) flown in the environment will be monitored. However, the final section labeled \emph{Test Flight} loosely describes the externally defined mission that will be deployed. This is interchangeable, as the platform user could execute many different missions in the same environment with goals of testing different types of behavior.  
\input{tables/tab_example_test}


\subsection{Configuration Parameters}
sUAS are particularly sensitive to their environments and therefore it is important to test them within context. As illustrated in our example, configurable parameters include weather, location, scene, and signal attributes. 





\subsubsection{Weather and Lighting Factors}
Weather conditions (wind, fog, rain), lighting conditions (sunny, dawn, dark),  radio interference, and continuous variation in GPS signal strength  greatly impact the functioning of both the UAV's perception of the environment and its control algorithms \cite{gao2021weather}, and thereby affect system safety. Wind speed is often cited as a cause of UAV crashes because high wind speed  in a particular direction can negatively affect the ability of the UAV to maintain its desired flight path \cite{lundby2019towards}. Furthermore, rain, fog, and snow, as well as low lighting conditions in the environment, impair the ability of computer vision models to interpret the environment correctly \cite{hamzeh2022improving}. Further, GPS signal quality continuously varies in the real world impacting autonomous navigation and autonomy computations, as discussed in \cite{Ankit's paper}. Therefore, \DW supports configuration and simulation of various weather conditions, and position of the sun (i.e., time of day) which creates various shades of lighting conditions.
\input{tables/tab_weather}

\subsubsection{Real World Location}
Standard UAV simulators such as Gazebo \cite{koenig2004design} include an empty environment or simple three-dimensional shapes such as cylinders and cubes as obstacles for UAVs to avoid. These simulation environments fail to capture the complexity of the shapes, sizes, textures, and terrains found in the real world. High-fidelity simulation environments that support rigorous integration and acceptance tests, need to incorporate real world environmental data.  This would allow test cases to validate whether a UAV can operate safely by avoiding trees or tall buildings, and whether it can plan routes that do not violate societal boundaries and impact individual privacy. Table \ref{tab:geo_props} shows examples of properties that can be configured into a simulated environment. These include the selection of digital twins of cities, safe landing stations within cities, restricted airspaces within the  cities for UAVs to avoid, and various  objects such as birds, pylons, and other flying vehicles. 
\jch{Needs to be a bit more substantiated with references from other simulation environments etc. We can also reference our own use cases (in 3rd person)}.
\input{tables/tab_realworld}

\subsubsection{Mission Specific Scenarios} The inclusion of custom landscapes and environments to support acceptance tests associated with realistic real-world scenarios is essential for testing the run-time behavior of the system as a whole. For example, the simulated environment for a UAV-supported river search and rescue operation could include a river, and an animation of a person struggling in the water with intermittently visible parts of their body as they move up the water level for a short amount of time before temporarily submerging. A simulation environment of this nature would test the effectiveness of integrating control algorithms, such as tracking or following the victim, with perception algorithms, such as detecting the victim.  Since designing such complex mission specific scenarios requires huge effort and time of UAV software developers, we aim to add landscapes and dynamic objects in support of extensive real-world scenarios into our simulation environment. UAV software developers will select scenarios and configure their properties to create customized simulations. Table \ref{tab:scenario_props} shows a subset of potential configurable properties for river search-and-rescue and fire surveillance missions. 
\input{tables/tab_scene}

\subsubsection{Signal and Interference}
\jch{@Ankit -- I think we can reference your (hopefully) new paper to talk about signal and HDOP. Also there was a talk at the Aviation/NASA conference about GPS loss behind buildings etc so I think we can set the scene here.} This section talks about wireless availability, interference, satellites (RTK option?), n3 (??) etc. the noise inherent to radio signal strength, and variations in GPS satellite count availability as summarized in Table \ref{tab:interference_feature}.
\input{tables/tab_signal}



\subsection{Human Interaction}
\jch{Something about human interactivity. I'm thinking (as per original test case example) that we might start simple and allow interactivity via RC and/or stream monitored data for the user application to use.)  Note: in our current deployment we already have some 'dangerous' human interactions, so we could mention these.  We crashed one drone based on this.}
\input{tables/tab_humans}


% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\columnwidth]{./figures/ENVFramework.drawio.png}
%     \caption{Overview of Categories in which  Environmental Properties and System Properties must be specified in order to design and generate  acceptance test artifacts. }
%     \label{fig:test_rules}
% \end{figure}
% Typo on "Environment PropOERties" \jch{Ankit I think the Flight and HoTL ones still need work. See this document: \url{https://docs.google.com/document/d/12WgCNnz_xCZ3HKj3Gcs03yKtEgv4PmivxT9E86plZXw/edit?usp=sharing}}

\section{Monitorable System Properties}
We leveraged three different sources of information to identify a set of sUAS-related safety properties which we monitor by default unless explicitly turned off by the user or irrelevant to the specific context. Several examples are shown in Table \ref{tab:example_spec}.

Our data sources included (1) a Systematic Literature Review (ask MV about the ones we ignored for our HIP FSE student because they weren't human related), (2) the section in sUAS documentation manuals describing emergency procedures as define a set of unwanted cases which need to be monitored for, with (3) the final list of properties augmented from our own domain knowledge of sUAS flying. 

Something about how users can augment properties.
\subsection{Runtime Monitoring}
How do we define them, monitor for them etc etc.




% \jch{The following needs replacing based on what we find from the above study.   }
% We also define a set of system properties specifying functional, safety, fairness, and usability qualities. Some system properties are expected to hold true across all acceptance tests, while others are applicable to specific tests.  As shown in  Figure \ref{fig:test_rules} we classify system properties into three primary categories of \emph{Mission} properties, \emph{HoTL}, and \emph{Perception} properties. 

% \subsection{Mission Properties}
% Mission properties are typically defined in terms of sensor data (e.g., GPS, gyroscopes, accelerometers, and magnetometers) which is indicative of UAV health throughout the mission, general mission information (e.g., separation distance between UAVs, ability to reach a safe landing station, authorized airspace, traversal of target waypoints), and control algorithms \cite{nguyen2020control} that define the run-time behavior of UAVs during a mission. 
% %Failure to acquire high-quality sensor data, communicate with other UAVs or software-based Ground Control Stations where  mission failure and compromise system safety. 
% Therefore, we have incorporated the following properties into our framework to support tests in different environmental configurations. 

% \noindent {\it S1: Flight:}
% In order to test the ability of the system to fly safely under a variety of environmental conditions, a complete mission is assigned to one or more UAVs. Tests based on flight properties validate whether UAVs in the mission are able to complete their assigned flight path under available resources such as battery, and whether they self-adapt their flight path as needed to complete the mission. \new{For example, in the \REALSIM environment, CPS developers could configure extreme windy conditions to test a UAV's capability to complete a mission. The run-time monitoring of battery voltage, vibration, and velocity would provide insights regarding a UAV's ability to fly successfully in real-world windy conditions.}

% \noindent {\it S2: Collision Avoidance:}
% \new{CPS developers impose multiple constraints on dynamically generated flight plans as well as UAV maneuvers to avoid collisions with} trees or buildings, other unmanned vehicles, and birds etc. Collision avoidance properties test whether the system constraints are sufficient to prevent collisions with objects in the environment, including other UAVs in the mission. \new{An example of a safety constraint for avoiding collisions is enforcing UAVs to maintain a minimum separation distance from other UAVs or objects in the environment. Test outcomes would enable developers or operators running preflight tests, to simulate a multi-UAV mission to verify whether the configured minimum separation distance is sufficient under extreme weather conditions, within a dense city environment, or in other specified operating environments. By monitoring run-time properties, such as the separation distance between the UAVs or the occurrence of actual collisions, would help validate the system design and support incremental improvements until tests passed consistently in anticipated operating conditions.}

% \noindent {\it S3: Restricted Airspace Avoidance:}
% During a mission, UAVs are prohibited from entering certain airspace in order to maintain air safety, as per FAA Guidelines. For instance, UAVs must avoid critical airspace such as class B airports and are prohibited from flying over landmarks such as stadiums, prisons, and hospitals. Furthermore, UAV operators typically create a safe geo-area in which UAVs are expected to remain in order to ensure mission safety. As a result, the Restricted Airspace Avoidance properties test whether the system is able to detect and avoid different restricted airspace in a variety of environmental conditions. For instance, developers could test whether a UAV is capable of avoiding restricted airspace when the GPS signal quality is very poor. Monitoring access to restricted airspace, UAV flight paths, and GPS signal quality would provide valuable insights into the system's ability to avoid restricted airspace in the real world.

% \subsection{HoTL Properties}
% Humans-on-the-Loop play a critical role in ensuring system safety, and humans and UAVs often need to collaborate on tasks together. Therefore, the HoTL properties of our framework specifically aim to test the Human-UAV interactions during an emergency response mission. These properties are derived from the primary goals of effective coordination and control between humans and machines namely  \textit{Transparency}, \textit{Augmented Cognition}, and \textit{Coordination} \cite{mcdermott2018human,cleland2022extending}. 

% \noindent {\it S4: Transparency:}
% As discussed in Chapter \ref{ch:chi2020}, situational awareness, defined at three different levels \cite{endsley2001designing} is crucial for effective Human-UAV partnerships. Further, in Chapter \ref{ch:autonomyExplanations}, we showed how \droneresponse provides necessary information in the form of explanations to keep humans aware of the situation. As a result, transparency properties, evaluated through user studies, test whether the system provides sufficient information about the environment and autonomous decision-making in various environmental conditions to keep humans sufficiently aware of the mission status.

% \noindent {\it S5: Augmented Cognition:}
% Automated UAVs are capable of adapting their plans, and requesting assistance from humans at different points in the mission in response to dynamic environmental changes. As discussed in Chapter \ref{ch:modre2020}, humans intervene into the UAV autonomy by providing \textit{feedback}, \textit{sharing knowledge} about the environment, and \textit{sending control commands}. These human interventions are generally intended to guide UAVs towards their mission objectives or to mitigate emergent hazards during the mission. The simulation environment enables user tests to validate whether the system provides users with capabilities and  opportunities to intervene in the autonomy of the UAVs when deemed necessary, under a variety of environmental conditions.

% \noindent {\it S6: Coordination:}
% During a mission, humans may acquire full manual control of an autonomous UAV to accomplish a task for a variety of factors such as the trustworthiness and reliability of the UAV in a specific mission scenario. Thus, the system relinquishes control of the mission to human users, and later, after obtaining permissions from humans, regains control. This notion of permission based autonomy control is discussed in Chapter \ref{ch:modre2020}). These properties are therefore designed to test the seamless transition of control between humans and UAVs during an emergency response.                                                                      

% \subsection{Perception Properties}

% Autonomous UAVs build their awareness of the environment using computer vision models  such as YOLO \cite{yolo_redmon2016you}. Failure to correctly recognize different elements of the environment cause UAVs' to behave unpredictably. Perception properties aim to test whether a UAV is capable of perceiving the environment correctly in various environmental conditions. 

% \noindent {\it S7: Confidence:}
%  As discussed earlier, the performance of a computer vision (CV) model is verified using images in the validation datasets, which may not represent all complexities of the environment. The differences between the validation datasets and real environmental conditions affect UAVs' perception, resulting in the system failure. In particular, the confidence metric of a model indicates the probability that it has recognized an element such as person, or birds in the environment correctly \cite{pouget2016confidence}. As a result, we included this property in our framework to test whether the computer vision model is capable of producing sufficient confidence under challenging environmental conditions or when used in multi-UAV scenarios in which UAVs may need to collaboratively agree and act upon their perceptions. Evaluating the use of CV models within simulation environments highlights the need for high-fidelity imagery.
 
% \noindent \textit{S8: Bias:}
% Computer vision models may be subject to bias due to their programming and data sources. As an example, a model may classify any person in the river as a drowning person. However, this is not always the case, as the UAV may have captured a person who was swimming in the river. The lack of swimmers in the data set on which the computer vision model is trained results in an inaccurate perception of the UAV. As a result, we included this property in our framework to test whether the UAV's perception is free from any possible bias or not. 


% % \jch{Ankit - maybe mention in 1-2 sentences that each system property is supported by one or more reusable test. For example, a system property stating that ``Minimum separation distance (MSD) must be maintained between all UAVs throughout the flight'' is supported by a dynamic test case that monitors distance between UAVs and fails when MSD is violated.}


% \section{Simulation Test Cases}

% \subsection{Test Case Specification}
% Given the available set of system properties and the configurable simulation environment, a developer (or dedicated tester) specifies an integration or acceptance test. The test includes three components: (1) a description of the mission or tasks to be performed by one or more UAVs, (2) a description of the simulation environment in which the mission is to be executed, and (3) a set of system properties that are expected to hold during the mission. Once the test case is written, the tester configures the simulation environment using the simulation configuration properties, defines a specific mission to be performed by one or more UAVs, and executes the test case by launching the mission and monitoring for any violations of system properties. We provide concrete examples of two tests that could be run in simulation to validate specific properties, in order to generate evidence of the system's safety. These tests align with the system properties shown in Figure \ref{fig:test_rules}.


% \begin{table}[htbp]
% \small
%     \centering
%     \caption{Simulating two different configurations of Environmental Features}
%     \label{tab:river_config}
%     \begin{tabular}{|c|c|c|}
%     \hline
%     \textbf{Environment Features}&\textbf{Configuration 1 (C1)}&\textbf{Configuration 2 (C2)} \\ \hline
% Environmental Factors&Wind = 23 mph & Rain = Heavy \\ \cline{2-3}
% & Time of Day = Afternoon&Time of Day = Evening \\ \hline
% Mission Specific Scen. &S= S\&R &S= S\&R \\ \cline{2-3}
% &River W= 10m, V=3mph, D=West& --- \\ \cline{2-3}
% &Victim A=20, G = M, H=5'10''&Victim A=50, G=F, H=5'10'' \\ \cline{2-3}
% &visible body part = Lower body&Visible body part = hands \\ \hline
% Geographic Sites&---&Region = Saint Joseph River \\ \hline
%     \end{tabular}
    
% \end{table}


% \begin{table}[htbp]
% \small
%     \centering
%      \caption{System Properties Under Test for two different environmental Configurations in the simulated Environment}
%     \label{tab:sys_props_river}
%     \begin{tabular}{|c|c|p{7cm}|c|}
%     \hline
%          \textbf{S. No} &\textbf{System Property}&{\multicolumn{1}{c}{\textbf{Example of a test}}} &\textbf{Env Config} \\ \hline
% S1&Flight & UAV battery never goes below 10\% during flight&C1, C2 \\ \hline
% S2&Collision Avoidance& UAV avoids collision with trees&C2\\ \hline
% S3&Airspace Avoidance& UAVs never enters any restricted airspace of a city&C2\\ \hline
% S4&Transparency& UAVs provide humans with sufficient and accurate explanations about mission status & C1, C2\\ \hline
% S5&Augmented Cognition& When UAVs track an object that is not a victim, human intervention to manually control the UAV is always successful & C1, C2\\ \hline
% S6&Coordination&UAVs avoid tracking objects that look like victims if they have previously been identified as “not victims” by a human operator. &C1, C2\\ \hline
% S7&Confidence& UAVs are capable of detecting a drowning individual in a river with a high degree of confidence (above 80 percent)&C1, C2\\ \hline
% S8&Bias& UAV is capable of detecting victims in the river regardless of their gender and visible body parts&C1, C2 \\ \hline
%     \end{tabular}
   
% \end{table}

% Each example shows a distinct configuration of the simulated environment. For example, configuration 2 (C2) represents the environmental conditions with the contextual information of: \textit{During heavy rain, around 5 PM at a section of the Saint Joseph River, a 50-year-old female of height 5'10'' has drowned and only her hands are visible.} Table \ref{tab:river_config} shows how each example is configured by setting simulation configuration properties in the simulator.



%  Table \ref{tab:sys_props_river} shows an example test for each system property in one or more environmental configurations. In practice, we would define a suite of tests for each type of property. For instance, S7 in Table \ref{tab:sys_props_river} examines whether a UAV can accurately detect a drowning person in both rainy and windy conditions. Similarly, S8 examines whether the UAV's computer vision model is biased against recognizing drowning victims of particular genders or not. Depending on the configuration of the environment, relevant properties of the system are chosen for testing. For instance, in Environmental Configuration C1 (Table \ref{tab:sys_props_river}), all properties are tested except for P3 (Restricted Airspace Avoidance) as the configured environment does not contain restricted airspace of a city, and P2 (under Collision Avoidance) since trees are not configured in the environment. All properties are tested for C2 (Table \ref{tab:river_config}), including P2 and P3, as the environment contains a region of a real city with trees.

%  \jch{Ankit: I think you need to just say, that you then plan an actual mission with UAVs, then all ubiquitous tests are activated, and mission-specific ones activated when relevant.  For example, in your table, tests associated with system properties 1, 4, 5, 6, 7, 8 are relevant to both tests, but S2 and S3 is only relevant to C2.  Actually, I would think 2 and 3 are also relevant to ALL.  If you have a single UAV example, and you have a property about UAV to UAV collisions, then that would be an example of a property that only activates under certain conditions.}

% As explained above, each of these proposed acceptance tests is supported by a suite of lower-level tests that check whether the relevant system properties hold throughout the test.



% \jch{MAJOR COMMENT HERE:  What yo need is a section on system properties with examples that map to the categories in Figure 1.1.  This should be separate from the scenarios.  In other words you need a section (which you have) that discussed the Simulation Configuration Properties, now you need a separate section on System properties, and FINALLY, you need a section that shows how both of these come together for specific scenarios.  You are missing the 'clean' and 'distinct' section on System properties (see the google sheet).}





% \begin{table}[htbp]
%     \centering
%     \caption{Configuration of Environmental Features to conduct simulation test for river search-and-rescue scenario}
%     \label{tab:river_env_config}
%     \begin{tabular}{|c|c|}
%     \hline
%          \textbf{Environment Features}	& \textbf{Configuration}  \\ \hline
%         \multirow{2}{*}{Environmental Factors}	& Wind=23 mph \\ \cline{2-2}
% 	& Time of Day = Afternoon \\ \cline{2-2}
% 	& GPS signal Quality = Good \\ \hline
% \multirow{4}{*}{Scenario Specific Component}& Scenarios = River Search and Rescue \\ \cline{2-2}
% 	& River Width = 10 m, Velocity=3mph, Direction=West \\ \cline{2-2}
% 	& Victim Age = 20, Gender = Male, Height=5'10'' \\ \cline{2-2}
% 	& Visible body part = Lower body \\ \hline
%     \end{tabular}
    
% \end{table}














% \subsection{Mission Properties}

% UAVs can complete a mission within the available battery power in foggy and dark weather conditions (\emph{Environmental Factor})
% UAVs can plan a safe route to deliver flotation devices (\emph{Mission Specific Scenarios})
% \noindent \textbf{S1: Individual / Multiple UAV Mission: } 


% In the context of river search-and-rescue missions, the simulation should demonstrate that (a) UAVs can complete a mission within the available battery power in foggy and dark weather conditions (\emph{Environmental Factor}), (b) UAVs can plan a safe route to deliver flotation devices (\emph{Mission Specific Scenarios}), and furthermore that (c) autonomous UAVs are capable of executing the mission in a realistic geographical location such as in a section of the St. Joseph River (\emph{Real Geographic Sites}). 

% \noindent \textbf{S2: Collision Avoidance:}

% In the context of a crime-surveillance mission, a test case in simulation could demonstrate that (a) UAVs are capable of avoiding collisions and re-planning their routes in conditions such as fog, snow, and rain, which have a direct impact on the visibility of UAVs (\emph{Environmental Factor}), (b) UAVs are capable of tracking a car driven at high speed by a criminal (\emph{Mission Specific Scenarios}), and (c) UAVs are capable of avoiding collisions with buildings and trees in a realistic city such as Boston or where the system is intended to be deployed (\emph{Real Geographic Sites}).    

%  \noindent \textbf{S3: Restricted Airspace Avoidance:}
 
%  The simulation test should demonstrate that (a) the system is capable of avoiding restricted airspace even if the GPS signal strength is not excellent (\emph{Environmental Factor}), (b) the system can detect a dense crowd at run-time and avoid flying over it  (\emph{Mission Specific Scenarios}), (c) UAVs can fly through a real geographic area while avoiding all the restricted airspace within the city (\emph{Real Geographic Sites}). 


 
 
% %  \subsection{Human-on-the-Loop Properties:}
 
 
% %  \noindent \textbf{S?: Transparency:}

 
% %  Therefore, the simulation tests should demonstrate that the system provides sufficient information regarding (a) the environmental conditions in which the UAV is operating, (b) automatically generated plans to achieve a mission-specific task, and (c) the geographical area in which a UAV is operating by using specific street names and landmarks of a city in the reasoning. During simulation tests, a human observer should monitor the autonomous mission through a graphical user interface, including aerial video streams, and verify that the system is transparent and provides sufficient information to understand the status of the mission. 

% % \noindent \textbf{S?: Augmented Cognition:}


% % For a river search-and-rescue mission, the simulation must demonstrate that (a) a human observer can quickly comprehend the weather alert provided by the UI (\emph{Environmental Factor}), analyze the aerial video stream to identify possible human actions, and intervenes into the UAV autonomy for safety, (b) human intervention in critical scenarios such as victim tracking, or flotation device delivery does not impact the expected functioning of onboard autonomy models (\emph{Mission Specific Scenarios}), and (c) humans are able to safely intervene to rescue a person from a realistic geographic site (\emph{Real Geographic Sites}). 

% % \noindent \textbf{S?: Coordination:}

 
% %  For example, consider that the UAV perceives a rock in the river as a potential drowning victim and switches to Tracking Mode. However, the human observer denies the presence of a victim and commands the UAV to change to Searching Mode. In this case, the UAV switches to Searching Mode for a few seconds, but once again identifies that rock as a victim and switches back to Tracking Mode (\emph{Mission Specific Scenarios}). Such runtime behavior causes system instability, resulting in mission failure. Similar tests can be conducted for various Environmental Factors and real-world Geographical configurations of the environment. 
 

% % \noindent \textbf{S6: AI Confidence:}
 
 
% %  When a computer vision model is used to recognize different elements of the environment, such as people, trees, buildings, or birds, the simulation test (i) should verify the model's confidence under different weather conditions (\emph{Environmental Factor}) is above a certain threshold, (ii) demonstrate that the model detects drowning individuals in a river flowing at high velocity, where only the lower portion of the individual can be seen through the UAV's camera  (\emph{Mission Specific Scenarios}), and (iii) the model's performance in a realistic geographical site would provide insight into whether the model's unpredictability is acceptable to deploy in the real world or not (\emph{Real Geographic Sites}). 

% % \noindent \textbf{S7: AI Biases:}
\subsection{Results Generation and Analysis}
UAV software consists of run-time monitoring programs for continuously observing and analyzing run-time behavior, including vehicle parameters, mission parameters, and autonomy model parameters. While we expect users of \REALSIM (e.g., Droneresponse developers) to independently monitor the runtime behavior of their own UAVs, we also plan to monitor this behavior directly in \REALSIM. Further, \REALSIM also monitors properties of the simulated environment to ensure that the simulation environment matches the specified test conditions, and to detect UAV interactions with the environment such as collisions with buildings, trees, or other UAVs. During the execution of each configured simulation, applicable system properties are monitored using  the monitoring capabilities of the UAV system and the simulation environment. If any  properties are violated then the violations are displayed and the test fails. The data collected from both the system monitors and the environment monitors can be synchronized by timestamps to automatically generate a simulation report that provides insight into the run-time behavior of the system to perform test diagnosis.

==> old/old_approach.tex <==
\section{\DW Architecture}
\label{sec:dr_architecture}
% \jch{This is where we describe the architecture of the \DW platform (NOT DroneResponse!!)}
We now present the architectural details of our multi-UAV platform, which we used to test our framework during the simulation testing phase.  A more complete description is provided in \cite{nafeeconfiguring2022}. The \droneresponse architecture is designed as a flexible and configurable framework for multi-UAV missions. Its architecture, shown in Figure \ref{fig:dr_arch}, has three main parts, each bearing a specific responsibility for planning, managing, and executing multi-UAV missions. 
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{./figures/System_Design.png}
    \caption{Components of \droneresponse Architecture}
    \label{fig:dr_arch}
\end{figure}
\subsection{User Interaction}
User interactions were a key driver during the design and development of \Droneresponse. The user-centric \textit{interfaces} allow stakeholders to configure missions, track sUAS, and monitor sUAS status on diverse devices such as laptops, tablets, and mobile phones. This flexibility is achieved via a centrally (cloud-)hosted \textit{web application}, and a dedicated \textit{database} for storing reusable mission plans and configurations, including search areas, flight paths, and sUAS roles.
The user interfaces follow a Model-View-Controller (MVC) pattern decoupling the presentation layer in order to reduce payloads for fast message exchange. The UI clients asynchronously send and receive data from an HTTP server which in turn processes data received from the Control Station message broker. Therefore, the HTTP server serves as a bridge for the User Interaction components to interact with the Coordination Services and UAV autonomy modules. Furthermore, the server also routes aerial video streams to the client applications. On the front-end, \droneresponse provides UI support for mission planning and progress tracking, sUAS tracking, monitoring of aerial video streams and POI markers. The design allows multiple users to work collaboratively in planning, communicating, and deploying missions, including tasks such as defining search areas and flight routes, configuring sUAS, and tracking missions.

\subsection{Ground Control Station} The Ground Control station in \droneresponse adheres to the microservices and publish-subscribe architectural style~\cite{muccini2018iot} with the aim of achieving scalable and lightweight mission-specific services. The \textit{Mission Coordinator} component consists of lightweight microservices -- each of which provides a specific capability such as airspace leasing, multi-sUAS coordination, or safety-checking the mission specification. 
In essence, each microservice is an abstraction of a specific mission functionality. Further, each microservice is designed independently and runs in parallel, with all services sharing access to  a run-time database for the exchange of time-sensitive sUAS information data, such as the last known location of an sUAS.  During a mission, microservices leverage messages received from the operator(s) and sUAS, along with this shared knowledge-base to support data-processing and decision-making. While some microservices are generic across all missions, others are configured with mission-specific capabilities. For example, in a river search-and-rescue mission, a microservice might be responsible for selecting an sUAS to track a victim, or in a pollution-sampling mission, a microservice might aggregate data from multiple sUAS to dynamically form a pollution map. Microservices make decisions which impact the actions of sUAS, and communicate these decisions in the form of control commands and messages via an MQTT message broker. Since the microservices are independent of each other, they can be deployed either locally, on a single machine, or on multiple cloud servers in a distributed manner to provide fault tolerance.



\subsection{UAV Onboard Autonomy} The \droneresponse system has a strong emphasis on UAV autonomy and onboard computation capabilities. This \textit{Autonomy} module is responsible for (a) supporting the autonomous behavior during the mission in conjunction with an Autopilot, (b) monitoring and processing necessary data to inform autonomous actions, and (c) collecting and broadcasting information across the team of sUAS and humans. The Onboard Autonomy model retrieves sensor data and sends commands to and from the flight controller via the connection layer. The \textit{Mission State} component dynamically generates mission-specific states, and transitions based on user-specified mission specifications at run-time that guides the autonomy of the sUAS during the mission. The \textit{Vision Model} component  processes the aerial video stream to detect objects of interest in the scene. This component is responsible for building the sUAS' perception of the environment, and adapting autonomous behavior such as re-planning routes to avoid collisions, adjusting the flying pattern based on weather conditions, and tracking a person.

\subsection{Implementation}
 For the implementation of our \droneresponse system, we utilized the MEAN stack (Mongo-Express-Angular-Node) as part of the  user interaction module. Angular~\cite{jain2014angularjs} is used as the web framework to implement the client application components, enabling a lightweight, platform-independent, single-page application. \textit{NodeJs} serves as the backend part, while \textit{Express} was used  to design the APIs for the client application to exchange data with the server. In case a stakeholder initiates a new connection request through a UI, \textit{NodeJs} proactively pushes all the data necessary to synchronize multiple instances of the UI clients. To achieve multi-client synchronization in close to real-time, \textit{NodeJs} establishes a connection with the \textit{MongoDb} \cite{mongodb} NoSQL database to store mission-specific data in the JSON format such as mission configuration, flight routes, search areas, and sUAS route assignments. In addition, \textit{NodeJS} contains two primary communication channels for sending and receiving data from other modules in our architecture. NodeJs instantiates an \textit{MQTT client} to publish and subscribe to messages from an \textit{MQTT broker}, in our case \textit{Mosquitto} \cite{mosquitto}, an open-source MQTT message broker. Secondly, \textit{NodeJs} utilizes web sockets to receive video stream data directly from each sUAS.
 
Microservices are implemented as independent Python modules containing MQTT clients to send and receive messages across the entire system using \textit{Mosquitto} in the control station. We utilized \textit{Redis} \cite{redis} for creating the run-time knowledge base of the control station, which is a distributed, in-memory key-value database proving real-time data management capabilities at scale and speed. 

In the Onboard Autonomy module, the message passing layer contains an MQTT client that publishes and subscribes messages to the message broker located in the Ground Control Station. This enabled the Onboard Autonomy module to communicate with micro-services and user interfaces. In addition, the message-passing layer contains a local MQTT broker and multiple clients that enable the components in the \textit{Autonomy Module} to exchange information with each other. The Autonomy modules uses the SMACH ROS package~\cite{smach} to implement a finite state machine that describes each UAVs' role in the mission based on the user-specified mission requirements. At run-time, the \textit{State Machine} component receives the mission specifications from the user via micro-services, and dynamically configures the valid states and allowed transitions for the sUAS whilst avoiding race conditions and deadlocks. These dynamically generated states and transitions govern the autonomous behavior of the UAV during mission execution. We used an off-the-shelf object detection AI model, called YOLO\cite{redmon2016you} to develop the computer vision component of this module. Finally, we used MAVROS \cite{mavros} ,which is a ROS package for communication over MAVLink protocol \cite{mavlink}, to send control commands from the Autonomy module to actuate the UAV. 

\section{Simulation Approach}
\label{sec:sim_approach}
This section explains our  approach for simulating the environmental features of our framework and its support for testing independent UAV applications such as the \droneresponse platform. 


The design of our simulation environment is inspired by the paradigm of game development. In order to generate a realistic testing environment, we used AirSim \cite{madaan_airsim_2020, shah2018airsim} and Unreal Game Engine \cite{unrealengine}. Figure \ref{fig:sim_approach} shows the overall architecture of the environment. 



\begin{figure*}[]
    \centering
    \includegraphics[width=\textwidth]{./figures/sim_arch_updated.png}
    \caption{UAV simulation in realistic environments}
    \label{fig:sim_approach}
\end{figure*}


\subsection{Environment}
As shown in Figure \ref{fig:sim_approach}, first, we used digital twins of popular cities to create a base layer of the environment consisting of 3D buildings with their actual heights and textures \textit{(Real World Geographic Sites)}. As a second step, we utilized animation features of the Unreal Engine to simulate dynamic aspects of the environment, such as a crowd in motion, a drowning person, or somebody running in order to evade police in a crowded city \textit{Mission Specific Scenarios}. In addition, we used Unreal's modeling features to simulate weather effects such as wind, rain, snow, and fog. The weather components allowed us to simulate challenging environmental conditions that directly affect the perception component of the Autonomy models. A user interface is provided to configure properties of each simulation feature of the environment prior to running a simulation test.

% Finally, we also included custom elements of the environment such as water flowing in a river with a specific velocity or smoke coming out of a window to reproduce mission-specific scenarios. 

\subsection{Flight Simulation}
We selected the Airsim simulator as our primary simulation tool for two primary reasons. First, Airsim is natively compatible with the Px4 Autopilot, on which our \droneresponse system is built. Second, Airsim is the only flight simulator that integrates with the Unreal Engine and is available as an open-source software system. On the left side of Figure \ref{fig:sim_approach}, we illustrate the integration of our \droneresponse system with the Airsim flight simulator. UAV onboard autonomy models send control commands via MAVLINK to the Px4 autopilot. In the Unreal Engine Game Environment, Airsim's Virtual UAV receives commands and actuation signals from the PX4 Autopilot to simulate the UAV in the configured environment.

\subsection{Human Interactions}
In order to support UAV software developers in testing HoTL properties of the system, we provide two channels for humans to interact. First, via the user interfaces of the \droneresponse system (DroneResponse UI discussed in Chapter \ref{ch:autonomyExplanations}, and Flying-AR discussed in Chapter \ref{ch:Human-UAV-Collaboration}), and second, via a handheld radio controller as shown in Figure \ref{fig:sim_approach}. This aspect of our simulation infrastructure is crucial for testing the HoTL properties \textit{(H5,H6)} of our framework. Current implementation of our simulation infrastructure supports human interactions via \droneresponse user interfaces, while interaction support via handheld controllers to fly a Px4 based UAV in Airsim is in development. 

\subsection{Geo-Reference Transformations}
Similar to popular flight simulation tools, such as Gazebo, Unreal Engine places objects in the environment based on Cartesian coordinates $(x,y,z)$ rather than the geo-coordinates (latitude, longitude, altitude) used by UAVs. Therefore, in order to place the digital twins of the cities in an unreal environment and fly multiple UAVs around them, we had to map the cartesian coordinate system and the geo-coordinate system in three dimensions. In order to address this particular challenge, we took advantage of the open source plugin known as CesiumForUnreal \cite{Cesiumfo86:online}. CesiumForUnreal enabled us to integrate an ellipsoid model of the earth into the Unreal environment and use its APIs to seamlessly transform positions between the Geo-Coordinate system and the Cartesian coordinate system. Using CesiumForUnreal, we added digital twins of cities to the elliptical model of Earth by transforming their geographical locations into Cartesian coordinates. In addition, we translate the real geolocation of the UAV into a Cartesian coordinate, so that the 3D model of the UAV can be placed in the Unreal environment at its real geolocation. Therefore, the geo-reference transformation plays an essential role in simulating the behavior of \droneresponse under realistic environmental conditions.


==> old/old_experiments.tex <==
\section{Experiments} 
\label{sec:sim_eval}

As an initial proof-of-concept, we demonstrated that the \REALSIM framework could support realistic tests of both single and multi-UAV missions using the \droneresponse platform under realistic environmental conditions.  In total, we conducted six different simulations to test the effects of wind, snow, and dark lighting conditions on the run-time behavior of UAVs during the Surveillance, Circular Pattern Flying, and AI-Driven Navigation phases of a mission inside digital twins of Boston, Melbourne, and Chicago.   




\subsection{Simulation Tests Descriptions}
 We configured two features of \REALSIM. These included  environmental factors to simulate weather conditions, and the use of geographic sites to add real world cities to the simulated environment. Additional configuration options, such as real-life scenarios, will be added over time. Table \ref{tab:sim_results} shows the configuration of the environmental features, \droneresponse mission type, and system properties tested in our proof-of-concept simulations.


\input{./tables/tab_simulation}

Test cases T1 and T2 validate UAV run-time behavior during a surveillance mission in which UAVs fly through a series of waypoints. In T-1, we checked whether UAVs are able to fly through each waypoint (S1:Flight) in windy \textit{(Environmental Factor)} conditions. T-1 is extended into T-2 by adding a real-world geographical environment, and checking whether one or more UAVs are able to navigate through each waypoint within the city of Boston \textit{(Real Geographic Sites)}. Due to the inclusion of a city in the environment, T-2 activates testing the S2 (Collision Avoidance) property of the system.

T-3 tests the run-time behavior of a UAV flying in a circular pattern. The UAV computes the circular path based on three input parameters: altitude, radius (from the home location), and velocity. We configured the environment to include Boston city and windy conditions. In our simulation test, we check if the UAV can complete its circular flight path \textit{(S1:Flight)} while avoiding collisions with nearby buildings \textit{(S2: Collision Avoidance)} under wind speeds of 20 mph from the east \textit{(Environmental Factor)}. 

T-4 and T-5 test the run-time behavior of UAVs under different lighting conditions. As a result, two environmental configurations of dark and light conditions in the city of Boston were selected. We checked whether a UAV can accurately use its AI-Driven navigation model \textit{(S7: Confidence)} to reach its target waypoint \textit{(S1:Flight)} while avoiding collisions with a building \textit{(S2: Avoid Collisions)}, both in normal and dark light conditions \textit{(Environmental Factors)}.  

\section{Analysis and Results of the Simulations}
% \jch{Start by summarizing results here} 
Results are summarized in Table \ref{tab:sim_results}, and indicate that three of the five tests executed successfully, whilst two resulted in collisions. We now describe our observations following the preliminary test.  

First, we observed that UAVs are capable of conducting the surveillance mission successfully in Boston (T1,T2) regardless of weather conditions. 

Second, our simulation approach revealed some interesting insights that would not have been possible with other popular simulators such as Gazebo. After the initial failure of T-3, the test analysis provided valuable information to determine the optimal parameter values for an algorithm that generates a circular flight path: the maximum altitude, maximum radius, and where to take off and land in order to fly in a circular pattern of radius 50 meters and an altitude of 20 meters from a location in downtown Chicago. Such insights could be very useful in conducting physical tests in the next phase of the development. The Figure \ref{fig:collision} illustrates how a UAV collided with a building while flying in a circular pattern of a radius of 20 meters from a specific location. 

Finally, conducting T-4 and T-5 simulation tests gave us greater insight into the performance of the AI-driven component in different lighting conditions. Figure \ref{fig:sun_pos} illustrates that the position of the Sun greatly influences the color and texture of buildings visible through the UAV camera, causing varying performance of the AI driven navigation. Accordingly, our simulation tests also provided insights regarding the time of the day when the uncertainty in the AI component is acceptable. The failure of T-5 suggests that physical tests should be carried out in bright light conditions before enhancing the AI model to perform equally well in darker light conditions. 



\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\columnwidth]{./figures/building_colission.png}
    \caption{The UAV Collides with a realistic building in the city of Boston during an Acceptance test of a control algorithm for flying the UAV in a circular pattern from a specific position in the city}
    \label{fig:collision}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\columnwidth]{./figures/sun_pos.png}
    \caption{Simulating Bright light and Dark Light area in a city based on the position of the sun}
    \label{fig:sun_pos}
\end{figure}

% \section{Results}
In summary, the results of our simulation tests provided valuable insights for designing and planning the physical testing in the real world. The successful execution of the \droneresponse missions using our  framework and simulation approach serves as an initial proof of concept that \REALSIM is useful for supporting high-fidelity realistic simulation testing for UAV applications during early stages of development. While we have currently tested only the S1, S2, and S7 system properties, and utilized Weather and Realistic Geographical Site features of our framework, the proof-of-concept simulations have shown the benefits of developing such a simulation environment. 

In order to evaluate mission-specific environmental constraints and HotL Properties (S4, S5, S6)  of our framework, we are working on creating animations of pertinent real-life rescue scenarios using the Unreal Engine and developing APIs to allow humans to intervene using a hand-held controller during simulation testing. 




















==> old_unused_drone_rescue.tex <==
Both use cases are enacted using our own semi-autonomous, multi-sUAS system~\footnote{name omitted due to double-anonymous review}, which includes a Ground Control Station (GCS) supported by a suite of microservices, autonomous processing capabilities located onboard each sUAS, and diverse GUIs to support human interactions. 

The Onboard Pilot acts as an application layer for the PX4 autopilot stack which includes flight control software and hardware for executing plans. Its internal \textit{State Machine} receives mission specifications and instantiates itself dynamically for the current mission. It then uses its onboard state machine to progress through a series of tasks, with transitions triggered by events it detects by analyzing its own sensor data and/or messages received from the GCS or other UAVs.

The ground control system uses microservices and a publish-subscribe architectural style~\cite{muccini2018iot}, with each microservice providing a specific capability such as airspace leasing, multi-sUAS coordination, or runtime monitoring. Finally, graphical and hardware user interfaces enable human-machine interactions. Most of the interactions are GUI-based; however, in case of emergency, humans can directly issue commands via hand-held radio controllers. The GUI components are built on a centrally hosted {\it web application} which asynchronously sends and receives status data and video streams over a mesh-radio via GCS's message broker and the onboard pilot modules.

%~\cite{ankit2021}. %Many of the runtime models are coupled with one or more GUIs that provide situational awareness to the human for planning and analysis purposes while also potentially monitoring aspects of human interaction behavior.

 %\vspace{-6pt}


==> sec_05_implementation.tex <==

%%%%%%%%%%%% MERGED INTO 3 and 5 %%%%%%%%%%%%%%%%%%%%%
%%% !!!!!!!!!!!!!!!!!! !!!!!!!!!!!!!!!!!!!!!!!!! %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Acceptance Testing \& \DW Implementation}
\label{sec:implementation}
In this section, we describe the Acceptance Tests and respective results provided by \DW and provide a brief overview of the current status of our prototypical implementation which is used in the subsequent experimental evaluation.

\subsection{Acceptance Tests and \DW Platform APIs}

As highlighted in the previous section, \DW collects runtime information from three primary sources, monitoring diverse sUAS sensors, the simulation environment, and human interactions with the sUAS. In order to be able to provide ``meaningful'' analysis and Acceptance Test results, it is necessary to provide additional information that goes beyond a simple \texttt{PASSED} or \texttt{FAILED} for a specific test.
For this purpose, \DW takes runtime information and consolidates them at the mission level from each sUAS in the environment, including any changes to the 3D environment.
This includes, for  example, \mv{add some example.} identifying whether two sUAS in the mission started tracking the same drowning victim in the river or not. 
Second, a  report is provided in if any of the test properties were breached during the mission. Test results are meant to provide key insights in how the mission was executed and in case of undesired behavior, explain \emph{how}, \emph{why}, and \emph{where} a specific test did fail. 
For example, in case where a lateral distance of is required and part of the acceptance test. An sUAS application developer excepts to be provided with detailed information on when this test fails. For example, at which point during the simulation was the distance constraint violated?, where in the simulation environment?, was any object hit as a result and what was the status of the sUAS at this point?  
With this information provided an sUAS developer can revisit the specified test case and analyze the behavior based on the timestamps provided and,  in case of a software  issue, trace the failure to a particular component in the sUAS application. For example, in case of distance violation the collision avoidance implementation may have provided inaccurate data, or was in turn provided with data unsuitable for calculating safe distances between two sUAS or an sUAS and an object in the environment. 

Given that the primary goal of \DW is to empower users to test diverse sUAS applications within various mission contexts, we created a number of extensible and  well-defined APIs which facilitate the easy adoption and interaction of  sUAS applications under test to interact with \DW.

 The APIs currently include a\\
  \emph{(1) Configuration API: } \DW provides end-users and developers with the ability to configure the environment and properties to be monitored. As an input, \DW accepts a JSON file structured as shown in Listings~\ref{lst:env_conf} and~\ref{lst:monitor_config}  to configure the simulation environment and monitor simulation results. \\
    \emph{(2) Application  Interface: } 
    In the sUAS software application development, the control commands are sent to the autopilot firmware, such as PX4, which generates the corresponding actuator signal and forwards it over a UDP or TCP connection to the simulator. Through DW, end-users can specify a unique port for each sUAS in the simulation to exchange data with the firmware, allowing seamless multi-sUAS simulations. \\
   \emph{ (3) Human Interaction Interface:} For the purpose of debugging and identifying the impact of human intervention on the runtime behavior of autonomous sUAS, \DW provides a virtual controller interface, which can be used to send control commands such as Take-off and Land or to switch sUAS modes. The virtual controller implementation may also be extended to physical controllers, as long as each key on the physical controller has a Python binding interface available.\\
   \emph{ (4) Simulation Data Subscription Service: } Finally, in order to enable developers to develop their own custom monitors, \DW publishes runtime monitoring data over MQTT topics to which developers can subscribe to monitor information about sUAS, environment, and human interactions. 
  
\subsection{Implementation}

For experimentation purposes with \DW (cf.~\citesec{sim_eval}), we implemented an initial prototype to support Pixhawk/PX4 application tests for a number of environmental configuration options and monitorable properties.
The configurable properties and features currently supported are marked as implemented (or partially implemented) in ~\citetable{factors}, and  monitors are further described in ~\citesec{sim_eval}.
Our \DW simulation environment was implemented using the Unreal Engine~\cite{unrealengine}, and  integrated open-source digital shadow models of the real world by using Cesium for Unreal~\cite {cesium}, a plugin for the Unreal Engine, to visualize and integrate high resolution, real-world, photogrammetry and 3D models.
For simulating sUAS we use  AirSim~\cite{shah2018airsim}, an open-source, cross-platform simulator for drones and several other types of (ground-based) vehicles.  Furthermore, we leveraged the APIs provided  by AirSim to simulate weather conditions in the environment, such as wind, fog, and snow. The simulation initialization manager component thereby instantiates multiple sUAS in the digital shadow of the real world and configures the environmental conditions as described in the test specifications. 
Finally, to collect, analyze, and validate the runtime behavior of sUAS and human interactions  \DW monitors were implemented as independent Python modules. These Python modules were configured and activated according to the test properties specified in the JSON file. To collect the different types of information necessary for validation three main types of monitors were implemented and used. First, monitors developed to capture the run-time behavior of suAS utilize AirSim's simulator APIs to directly connect to the (simulated) sUAS and to query data. Second, the human interaction monitor established a connection with the input devices, such as UIs, RC handheld controllers, keyboards, or game controllers, to record human interactions during mission execution. Finally, we used ``Unreal Blueprints'' to monitor the changes in the environment as well as the activities of a specific actor in it. For example, a drowning victim or an escaping suspect. Unreal Blueprint is a visual scripting technology that allows us to monitor and control every element in the Unreal Environment, recording a corresponding timestamp for each collected information. This is later vital for consolidating the data based on timestamps and generate the final test report. 

With regards to acceptance tests, we currently provide a textual output of these results on the command-line of the monitoring and simulation environment and in a log report. However, as part of our ongoing effort, we are currently working on a proper user interface Dashboard for providing visual (runtime) information and live updates to the user during test execution.




==> tables/backup_factors.tex <==
\begin{table*}[]
    \centering
     \addtolength{\tabcolsep}{-3.2pt}
     \caption{Configurable Properties}
    \label{tab:factors}
    \begin{tabular}{|L{1.4cm}|L{4.8cm} |L{3.9cm}|L{6.5cm}|c|}
     \hline
{\bf Category}&{\bf Observed Incidents}&{\bf Feature}& {\bf Configuration Parameters}& \\ \hline
\multirow{3}{*}{Scene} & \multirow{3}{*}{
\begin{minipage}[c]{4.4cm}
sUAS hitting immovable objects, such as buildings or rocks, and interfering with air traffic and humans on the ground~\cite{Incident-Balloon} ~\cite{CONFIG-L4}~\cite{CONFIG-L2}~\cite{CONFIG-L3}.
\end{minipage}
}
  &Regions& Region Name, Central coordinates (LLA)& \CIRCLE\\ \cline{3-5}
& &Terrain type& Mountainous, Forrested, River, Ocean, Urban.& \Circle\\ \cline{3-5}


& &Scene& Examples: Air Traffic, Crowd, Ground traffic, accident, building fire etc.& \Circle\\ \hline

GPS&  

\multirow{2}{*}{
\begin{minipage}[c]{4.4cm}
sUAS losing GPS signal or experiencing low GPS accuracy during flight~\cite{CONFIG-S1}.
\end{minipage}
}

& Degree of GPS deprivation& [0-100\%]& \Circle\\ \cline{3-5}
& & GPS availability plugin& [RandomDisturbance, GNSSModel]& \Circle\\ \hline


Weather \& Lighting&

\multirow{2}{*}{
\begin{minipage}[c]{4.4cm}
sUAS being blown off course due to high winds, operating outside its capabilities, or suffering mechanical issues due to environmental conditions~\cite{CONFIG-W2}.
\end{minipage}
}

& Weather conditions& [Sunny, Cloudy, Raining (heavy, medium, low), Snowing (heavy, medium, low)]& \RIGHTcircle\\ \cline{3-5}
&& Lighting conditions& dawn, morning, afternoon, dusk, night& \CIRCLE\\ \cline{3-5}
&& Temperature& [Celsius (-30-40), Fahrenheit (-20-120)]& \Circle\\ \cline{3-5}
&& Wind& For each range [altitude(upper, lower),wind speed (mph), wind gusts (mph), direction]& \CIRCLE\\ \hline
Human Interactions&

\multirow{2}{*}{
\begin{minipage}[c]{4.4cm}
sUAS not being operated correctly; issues related to unclear/ambiguous user interfaces~\cite{Incident-Balloon}.
\end{minipage}
}


&Mapping RC signals to DroneWorld's expected inputs. \newline & Examples:
Mode switches (e.g., Loiter, Stabilize, RTL, LAND)
Gimbal \& Camera controls& \RIGHTcircle\\ \hline
Sensors and Hardware &

\multirow{2}{*}{
\begin{minipage}[c]{4.4cm}
sUAS losing battery power mid-flight; damage to motors or other critical parts~\cite{Incident-Bat1},\cite{Incident-HW1},  \cite{CONFIG-F1}.
\end{minipage}
}

&Fault injection model& Fault Model Name,
Fault Types e.g., [Loss of signal, Magnetic Interference, Vibration etc]. \newline & \Circle\\ \hline
    \end{tabular}
    \DW Status: \CIRCLE=Implemented; \RIGHTcircle=Partially implemented;  \Circle=Not yet Implemented
\end{table*}


==> tables/monitors.tex <==
\begin{table*}[htbp]
    \centering
    \begin{tabular}{|c|L{7.5cm}|L{7cm}|}
        \hline
        \textbf{Monitor Name} & \textbf{Description} & \textbf{User Configurable Properties} \\ 
        \hline
        Horizontal Distance & Monitors the horizontal seperation between all sUAS in the misssion&  Minimum seperation distance (in meters) \\  \hline
        Lateral Distance & Monitors the lateral seperation between all sUAS in the misssion&  Minimum lateral seperation distance (in meters) \\  \hline
         Landing Spots & Monitors whether sUAS lands only in safe landing spots &  Number of safe landing spots and their geolocations\\  \hline
         No Fly Zone & Monitors whether sUAS enters in to any No Fly Zone areas & Number of no fly zones and geographic polygon for each zone \\ \hline
         Flight Trajectory & Monitors the drift in the flight trajectory & Maximum Acceptable drift in the flight path (in meteres) \\  \hline
        Collision & Monitors collisions with sUAS and environmental elements during the mission & NA \\ \hline
        Ordered Waypoint & Monitors Whether sUAS managed to reach their waypoints in order of assignment & NA \\ \hline
        Waypoint Precision & Monitors the precision with which sUAS achieved all assigned waypoints & Maximum acceptable deviation (in meters) when reaching a waypoint \\ \hline 
        Human Intervention & Monitors commands sent by human operator during the mission & Configure the controller type and settings \\ \hline 
         
         
         
         
    \end{tabular}
    \caption{\DW users can configure the characteristics of monitors to suit their needs for testing and analysis}
    \label{tab:monitors}
\end{table*}


==> tables/tab_configurable_properties.tex <==
\begin{table}[!b]
    \centering
     \addtolength{\tabcolsep}{-4.2pt}
     \caption{Configurable Properties}
    \label{tab:allprops}
    \begin{tabular}{|L{1.2cm}|L{2.8cm}|L{3.8cm}|c|}
     \hline
{\bf Category}&{\bf Feature}& {\bf Configuration Parameters}& \\ \hline
\multirow{3}{*}{\bf Location}&Regions& Region Name, Central coordinates (LLA)& \CIRCLE\\ \cline{2-4}
&Terrain type& Mountainous, Forrested, River, Ocean, Urban.& \Circle\\ \cline{2-4}
&Scene& Examples: Air Traffic, Crowd, Ground traffic, accident, building fire etc.& \Circle\\ \hline
{\bf GPS}&Degree of GPS deprivation& [0-100\%]& \Circle\\ \cline{2-4}
&GPS availability plugin& [Random, SatelliteComputed]& \Circle\\ \hline
Weather \& Lighting&Weather conditions& [Sunny, Cloudy, Raining (heavy, medium, low), Snowing (heavy, medium, low)]& \CIRCLE\\ \cline{2-4}
&Lighting conditions& dawn, morning, afternoon, dusk, night& \CIRCLE\\ \cline{2-4}
&Temperature& [Celsius (-30-40), Fahrenheit (-20-120)]& \Circle\\ \cline{2-4}
&Wind& [steady mph, gusts mph, direction, altitude range]*& \CIRCLE\\ \hline
Human Interactions&Mapping RC signals to DroneWorld's expected inputs.& Examples:
Mode switches (e.g., Loiter, Stabilize, RTL, LAND)
Gimbal \& Camera controls& \CIRCLE\\ \hline
Sensors \& Hardware &Fault injection model& Fault Model Name,
Fault Types e.g., [Loss of signal, Magnetic Interference, Vibration etc]& \Circle\\ \hline
    \end{tabular}
    \DW Status: \CIRCLE=Implemented; \Circle=Not yet Implemented
\end{table}

==> tables/tab_example_test.tex <==
\begin{table}[]
    \centering
    \caption{An example test case specifying meta-data, mission characteristics, environment, and safety properties to be checked. \jch{Formalize the safety properties a bit more. Maybe move this after everything has been defined.  This NEEDS to match whatever we define.}}
    \label{tab:example_spec}
    \begin{tabular}{|L{1.5cm}|L{6.5cm}|}
    \hline
         \multicolumn{2}{|c|}{\bf Test Description}\\ \hline
         Test ID & TST-0023\\ \hline
         Test Name&Boston in Windy Conditions \\ \hline
         \multirow{3}{1.5cm}{Test Description}& A UAV shall successfully complete a mission consisting of a series of waypoints in high wind conditions at 23 mph for altitudes above 30ft AGL.\\ \hline
    
           \multicolumn{2}{c}{} \\ \hline
         \multicolumn{2}{|c|}{\bf Configuration Parameters} \\ \hline
         \multirow{4}{1.5cm}{Weather}& (wind=15mph, $0<ALT<30ft$ AGL)\\
         & (wind = 23mph,$ALT>30ft$ AGL)\\
         &(precipitation=none, clouds=none,sunshine=bright)\\ 
         &(timeOfDay=Dawn)\\\hline
         \multirow{2}{1.5cm}{Location}&(Region=Boston Downtown)\\
         & (Central Point=(42.358564, -71.057413))\\ \hline
         \multirow{2}{1.5cm}{Scene}&(AirTraffic=None)\\ 
         &(Pedestrians=Random,GroundTraffic=Light, CarAccident=True,(COORDINATES))\\ \hline
         \multirow{2}{1.5cm}{Signal}&(RadioInterference=none)\\
         &(GPS:15 Satellites, GPSDeadSpots:None)\\ \hline
          \multirow{2}{1.5cm}{Human Factors}&Interactive\_RadioController [True,False]\\
         &Situational\_Awareness\_Data\_Streamed [True,False]\\ \hline
         \multicolumn{2}{c}{} \\ \hline
         \multicolumn{2}{|c|}{\bf Monitorable Safety Properties (Examples only)} \\ \hline
         \multirow{5}{1.5cm}{Default sUAS properties} &$\checkmark$~~sUAS eventually returns home with battery $> 20\%$\\
         &$\checkmark$~~sUAS always remains in authorized airspace\\
         &$\checkmark$~~sUAS does not collide with buildings\\
          &$\checkmark$~~Continuous L2 comm signal failure $< 30$ seconds\\ 
         &$\checkmark$~~Minimum sUAS separation distance is not violated\\ \hline
          \multirow{2}{1.5cm}{Mission Specific Properties}&$\checkmark$~~sUAS maintain lateral separation at all times\\ 
          &$\checkmark$~~sUAS do not violate Boston downtown speed constraints.\\ \hline
         \multicolumn{2}{c}{} \\ \hline
         \multicolumn{2}{|c|}{\bf Example Test-case Flights} \\ \hline
         \multirow{2}{1.5cm}{Test 1:}&AccidentSurveillance-002.flt \\
         &1 hexcopter dispatched for traffic accident surveillance \\\hline
         \multirow{2}{1.5cm}{Test 2:}&PollutionMonitoring-314.flt \\
         &4 hexcopters perform pollution monitoring task \\\hline
        \end{tabular}

\end{table}

==> tables/tab_humans.tex <==
\begin{table}[htbp]
    \centering
   \caption{Configurable Human Interactivity Factors. \jch{Fix!!}}
       \addtolength{\tabcolsep}{-4.4pt}
    \begin{tabular}{|L{1.5cm}|L{6.7cm}|c |}
     \hline
        \multirow{2}{1.5cm}{\bf Something} & Something [X,Y] &\CIRCLE \\ 
         &Something\_else [A,B,C]&\CIRCLE \\\hline
          
    \end{tabular}
    \begin{tablenotes}
    \item ~~~~\CIRCLE=Implemented; \RIGHTcircle=Partially Implemented; \Circle=Not integrated
    \end{tablenotes}
    
    \label{tab:interference_feature}
\end{table}

==> tables/tab_realworld.tex <==
\begin{table}[htbp]
    \centering
   \caption{Configurable Real World Location \jch{Add missing stuff}}
    \addtolength{\tabcolsep}{-4.4pt}
    \begin{tabular}{|L{1.5cm}|L{6.7cm}|c |}
     \hline
        \textbf{Category} & \textbf{Configurable Properties}& \\ \hline
          \multirow{2}{1.5cm}{\bf Location} & Coordinates [Lat, Long] &\CIRCLE \\ 
         &Location\_Type [City, Suburbs, Rural]&\CIRCLE \\\hline
        %  Safe Landing Stations & Count, Lat, Long \\ \hline
        %  Hazardous Area & Count, shape, (lat, long) \\ \hline
        %  Objects & Birds, Geese, Manned and Unmanned Vehicles, \\ \hline
     \end{tabular}
    \begin{tablenotes}
    \item ~~~~\CIRCLE=Implemented; \RIGHTcircle=Partially Implemented; \Circle=Not integrated
    \end{tablenotes}
    
    \label{tab:realWorld}
\end{table}


% \begin{table}[htbp]
%     \centering
%     \caption{Configurable Properties of the real world in simulation}
%     \begin{tabular}{|c|c|}
%     \hline
%          \textbf{Real world Components} & \textbf{Configurable Simulation Properties}  \\ \hline
%          Geographical Area & City, (Lat, Long)  \\ \hline
%          Safe Landing Stations & Count, Lat, Long \\ \hline
%          Hazardous Area & Count, shape, (lat, long) \\ \hline
%          Objects & Birds, Geese, Manned and Unmanned Vehicles, \\ \hline
         
%     \end{tabular}
    
%     \label{tab:geo_props}
% \end{table}

==> tables/tab_scene.tex <==
\begin{table}[htbp]
    \centering
   \caption{Configurable Scenarios \jch{Add missing stuff}}
    \addtolength{\tabcolsep}{-4.4pt}
    \begin{tabular}{|L{1.5cm}|L{6.7cm}|c |}
     \hline
        \textbf{Category} & \textbf{Configurable Properties}& \\ \hline
          \multirow{2}{1.5cm}{\bf Something} & Something [X,Y] &\CIRCLE \\ 
         &Something\_else [A,B,C]&\CIRCLE \\\hline
        %  Safe Landing Stations & Count, Lat, Long \\ \hline
        %  Hazardous Area & Count, shape, (lat, long) \\ \hline
        %  Objects & Birds, Geese, Manned and Unmanned Vehicles, \\ \hline
     \end{tabular}
    \begin{tablenotes}
    \item ~~~~\CIRCLE=Implemented; \RIGHTcircle=Partially Implemented; \Circle=Not integrated
    \end{tablenotes}
    
    \label{tab:realWorld}
\end{table}


% NEeds fixing

% \begin{table}[htbp]
%     \centering
%     \caption{Scenario Specific Configurable Properties}
%     \small
%     \addtolength{\tabcolsep}{-1.56pt}
%     \begin{tabular}{|c|c|c|}
%     \hline
%          \textbf{Scenarios} & \textbf{Scenario Components} & \textbf{Configurable Properties} \\ \hline
%          \multirow{4}{*}{River Search \& Rescue}& River & Width, Velocity, direction \\ \cline{2-3}
%         %  &Water Stream &  \\ \cline{2-3}
%          &Victim physical attributes & Age, Gender, Skin Color, Height \\ \cline{2-3}
%          &Visible body parts & Hand, head, upper body, lower body \\ \hline
         
%          \multirow{2}{*}{Fire Surveillance} & Entity & House, Building, Forest \\ \cline{2-3}
%          & Env Characteristic & Open Fields, Dense \\ \cline{2-3} 
%          & Fire Severity & Smoke, Light Flames, Burned \\ \hline
         
         
         
%     \end{tabular}
    
%     \label{tab:scenario_props}
% \end{table}

==> tables/tab_signal.tex <==
\begin{table}[htbp]
    \centering
   \caption{Configurable Communication and Signal Factors. \jch{Fix!!}}
       \addtolength{\tabcolsep}{-4.4pt}
    \begin{tabular}{|L{1.5cm}|L{6.7cm}|c |}
     \hline
         Satellite & Satellite availability& \Circle\\ \hline
         Signal Quality & Signal strength, Interference& \Circle \\ \hline
          
    \end{tabular}
    \begin{tablenotes}
    \item ~~~~\CIRCLE=Implemented; \RIGHTcircle=Partially Implemented; \Circle=Not integrated
    \end{tablenotes}
    
    \label{tab:interference_feature}
\end{table}

==> tables/tab_simulation.tex <==
\begin{table}[htbp]
    \centering
      \caption{Environmental conditions and system properties under test in the simulation}
    \label{tab:sim_results}
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
        \textbf{No.} & \textbf{Env. Factor}  & \textbf{Real Geo.} & \textbf{DR Mission Type} & \textbf{Sys Prop.} & \textbf{Result}  \\ \hline
         T-1&Wind & &  Surveillance &  S1 & Success\\ \hline  
         T-2& &  Boston&   Surveillance & S1, S2& Success \\ \hline  
        %  T-3&Snow  & Melbourne &  Surveillance & S1, S2 & Success  \\ \hline  
         T-3&Wind  & Boston & Pattern Flying & S1, S2 & Collisions detected\\ \hline  
           T-4 && Boston &  AI-Driven Nav. & S1, S2 & Success \\ \hline
           T-5& Dark lights & Boston &  AI-Driven Nav. & S1, S2, S7 &  Collisions Detected\\ \hline
    \end{tabular}
  
\end{table}

==> tables/tab_weather.tex <==
\begin{table}[htbp]
    \centering
   \caption{Configurable Weather and Lighting Factors}
    \addtolength{\tabcolsep}{-4.4pt}
    \begin{tabular}{|L{1.5cm}|L{6.7cm}|c |}
     \hline
        \textbf{Category} & \textbf{Configurable Properties}& \\ \hline
         \multirow{3}{1.5cm}{\bf Wind}& Wind\_Speed [0-40mph,Altitude\_Range[0-1000Ft AGL]]&\CIRCLE\\
         & Wind\_Gusts [0-40mph,Altitude\_Range[0-1000Ft AGL]]&\CIRCLE\\
         &Wind\_Direction [N,NE,E,SE,S,SW,W,NW]
         &\CIRCLE\\ \hline%, Region, Intensity \\ \hline
          \multirow{2}{1.5cm}{\bf Precipi-tation}&Precipitation\_Type [Snow, Rain, Fog]&\RIGHTcircle\\ 
         &Precipitation\_Severity[Light, Medium, Heavy]&\Circle\\ \hline
         {\bf Visibility}&Visibility\_Distance [0.0-5.0Miles] &\Circle\\ \hline
         {\bf Lighting} & Time\_Of\_Day [Daylight, Dawn, Dusk, Night]&\RIGHTcircle \\ \hline
     \end{tabular}
    \begin{tablenotes}
    \item ~~~~\CIRCLE=Implemented; \RIGHTcircle=Partially Implemented; \Circle=Not integrated
    \end{tablenotes}
    
    \label{tab:interference_feature}
\end{table}
